A General framework for PAC-Bayes Bounds for Meta-Learning

Meta learning automatically infers an inductive bias, that includes the hyperparameter of the base-learning algorithm, by observing data from a finite number of related tasks. This paper studies PAC-Bayes bounds on meta generalization gap. The meta-generalization gap comprises two sources of generalization gaps: the environment-level and task-level gaps resulting from observation of a finite number of tasks and data samples per task, respectively. In this paper, by upper bounding arbitrary convex functions, which link the expected and empirical losses at the environment and also per-task levels, we obtain new PAC-Bayes bounds. Using these bounds, we develop new PAC-Bayes meta-learning algorithms. Numerical examples demonstrate the merits of the proposed novel bounds and algorithm in comparison to prior PAC-Bayes bounds for meta-learning.

==> textfile/Original_complex.tex <==

\section{General Approach for Meta Learning}
\label{gen_sec}
In this section, firstly, we find a  general bound like \cite[Theorem 2]{omar} for the meta-generalization gap defined in the row $9$th of Table \ref{table_notation}. To do this,  let $\PriorTsk$  and $\PriorEnv$ denote the prior distributions at the task and environment levels, respectively. From the row $17$th of Table \ref{table_notation}, we recall that 
$\PriorTsk$  and $\PriorEnv$  can denote both data-free or data-dependent priors.
 Proposition \ref{prop-gen-pac-tsk} and Proposition \ref{prop-gen-pac-env} give similar bound like \cite[Theorem 2]{omar} at the task and environment levels, respectively.  


Now, in view of \eqref{decom-pac}, we continue with the following propositions.

\begin{proposition}
\label{prop-gen-pac-tsk}
Let $\funcTsk[a]{b}$ be a function which is convex in both $a$ and $b$. For any data-free or data-dependent prior $\PriorTsk$, with probability at least $1-\delta_i$ under $\mathrm P_{\trainTsk}$,  we have
\begin{align}
 \funcTsk[\mathbbm E_{\PWcondZimU}(\expLossTskRV)]{\mathbbm E_{\PWcondZimU}(\empLossTskRV)}\hspace{10em}\nonumber\\
 \leq   
 \Dkl\left(\PWcondZimU||\PriorTsk  \right)
+\log\left(\frac{
\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right),
\label{prop-gen-pac-tsk_formula}
\end{align}
where $\theta\in\mathbbm R^+$.
%Additionally, if the loss function is bounded on the interval $[\phi_{\min},\phi_{\max}]$, with probability at least $1-\delta_i$ under $\mathrm P_{\trainTsk}$,  we have
%\begin{align}
% \theta\funcTsk[\mathbbm E_{\PWcondZimU}(\expLossTskRV)]{\mathbbm E_{\PWcondZimU}(\empLossTskRV)}\leq\min_{\alpha\in[0,1]}   
% \Dkl\left(\PWcondZimU||\PriorTsk  \right)\nonumber\\
%  -\DAre[\alpha]{\PWcondZimU}{\PriorTsk}
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\theta\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right),
%\end{align}
%where $\DAre[\alpha]{}{}$ is defined by \eqref{newOne}.
\end{proposition}
\begin{proof}
\begin{align}
       &\funcTsk[\mathbbm E_{\PWcondZimU}(\expLossTskRV)]{\mathbbm E_{\PWcondZimU}(\empLossTskRV)}\\
        %%%%%%%%%%%%%%%%%%%%%%%%%line2
\textup{Jensen's Inequality} \hspace{2em}       &\leq 
\mathbbm E_{\PWcondZimU}\funcTsk[\expLossTskRV]{\empLossTskRV}
\\
        %%%%%%%%%%%%%%%%%%%%%%%%%line3
\textup{Eq. \eqref{Donsker} or \eqref{newOne}}  \hspace{2em} 
   &\leq 
\Dkl\left(\PWcondZimU||\PriorTsk  \right)
+\log\left(
\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}\right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\line4
\textup{Markiv; w.p. $\geq 1-\delta_i$}\hspace{2em}
&\leq 
\Dkl\left(\PWcondZimU||\PriorTsk  \right)
+\log\left(\frac{
\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right).
\end{align}
\end{proof}
\begin{proposition}
\label{prop-gen-pac-env}
Let $\funcEnv[a]{b}$ be a function which is convex in both $a$ and $b$. For any data-free or data-dependent prior $\PriorEnv$, with probability at least $1-\delta_0$ under $\mathrm P_{\trainEnv}$,  we have
\begin{align}
\funcEnv[\mathbbm E_{\hyperpost}\big(\expLossEnvRV\big)]{\mathbbm E_{\hyperpost}\Big(\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV\Big)}\hspace{10em}\nonumber\\
\leq \mathbbm E_{\hyperpost} \left(
\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}
\right)\label{Pr_env1}
\\
 \leq   
 \Dkl\left(\hyperpost||\PriorEnv  \right)
+\log\left(\frac{
\mathbbm E_{\mathrm P_{ \trainEnv}}\mathbbm E_{\PriorEnv}\, e^{\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}}}{\delta_0}\right),\label{Pr_env}
\end{align}
where $\theta\in\mathbbm R^+$.
%Additionally, if the loss function is bounded on the interval $[\phi_{\min},\phi_{\max}]$, with probability at least $1-\delta_i$ under $\mathrm P_{\trainEnv}$,  we have
%\begin{align}
% \theta\funcEnv[\mathbbm E_{\hyperpost}(\expLossEnvRV)]{\mathbbm E_{\hyperpost}(\empLossEnvRV)} \leq   \min_{\alpha\in[0,1]}
% \Dkl\left(\hyperpost||\PriorEnv  \right)\nonumber\\
%-\DAre[\alpha]{\hyperpost}{\PriorEnv}
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainEnv}}\mathbbm E_{\PriorEnv}\, e^{\theta\funcEnv[\expLossEnvRV]{\empLossEnvRV}}}{\delta_0}\right)
%\end{align}
%where $\DAre[\alpha]{}{}$ is defined by \eqref{newOne}.
\end{proposition}
\begin{proof}
The proof is very similar to the proof of Proposition \ref{prop-gen-pac-tsk}. 
\end{proof}

Next, by combining Propositions \ref{prop-gen-pac-tsk} and \ref{prop-gen-pac-env}, we can obtain  PAC-Bayes bounds for the meta-learning problem. To find such bounds, we need additional tools.
In the following, we present lemmas, which are used to derive PAC-Bayes bounds for the meta-learning problem.
\begin{lemma}
\label{Lemma_sum}
Let $X_i$ for  $i=1,...,\lenDataSet$ be independent random variables. Suppose  that for given $a_i\in\mathbbm R^+$, and  measurable  function $f_i$
\begin{align}
    \mathbbm P_{X_{i}}[f_i(X_i)\geq a_i]\leq \delta_i,\label{2020.08.05_19.45}
\end{align}
where $\delta_i\in[0,1]$. Then, 
\begin{align}
    \mathbbm P_{X_{1:\lenDataSet}}\left[\sum_i f_i(X_i)\leq \sum_i a_i\right]\geq 1-\sum_i\delta_i.\label{2021.02.21_23.11}
\end{align}
\end{lemma}
\begin{proof}
Firstly, we show that
\begin{align}
   \underbrace{ \left\{(x_1,...,x_\lenDataSet):\; \sum_i f_i(x_i)\geq  \sum_i a_i\right\}}_{\mathcal A}\subseteq\underbrace{\bigcup_{i=1}\{x_i:\; f_i(x_i)\geq a_i\}}_{\mathcal B}.\label{2021.02.21_23.12}
\end{align}
Let $(x_1,...,x_\lenDataSet)\notin \mathcal B$. It means that for all $i=1,...,\lenDataSet$, $f_i(x_i)<a_i$ which leads that $\sum_i f_i(x_i)<\sum_i a_i$, or $(x_1,...,x_\lenDataSet)\notin \mathcal A$. Thus, $\mathcal B^c\subset \mathcal A^c$, or equivalently $\mathcal A\subset \mathcal B$.

Next, from \eqref{2021.02.21_23.12}, one can conclude
\begin{align}
    \mathbbm P_{X_{1:\lenDataSet}}\left[\sum_i f_i(X_i)\geqslant \sum_i a_i\right ]\leq
    \sum_i     \mathbbm P_{X_{1:\lenDataSet}}\left[  f_i(X_i)\geqslant  a_i\right ]=    \sum_i     \mathbbm P_{X_{i}}\left[  f_i(X_i)\geqslant  a_i\right ]
    \leq\sum_i\delta_i \label{2020.08.05_19.58}
\end{align}
where the last inequality follows from
\eqref{2020.08.05_19.45}.  The proof can be concluded from \eqref{2020.08.05_19.58}.

\end{proof}


\begin{lemma}
\label{lem_triangle}
Let $\func[]{}$ be a function satisfying the following  inequality
\begin{align}
  \func[x]{y}\leq a_1 \cdot \func[x]{z}+ a_2 \cdot \func[z]{y}, \label{2021.02.21_22.34}
\end{align}
where $a_1$ and $a_2$ are positive coefficient. 
Under probability $\mathrm P_{\trainEnv}$, we have
\begin{align}
    \mathbbm P\left( \mathbbm E_{\hyperpost} \left[\func[\expLossEnvRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}
        +
        \textup{B}_{\textup{e}}\right)\hspace{5em}\nonumber\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \leq
            \mathbbm P\left(a_1\cdot \mathbbm E_{\hyperpost} \left[\func[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMeta[U]{\bm Z^\lenZm_i}{\task_i}}  \right]\geq        \textup{B}_{\textup{e}}\right)\nonumber\\
            +
                  \mathbbm P\left( a_2\cdot\mathbbm E_{\hyperpost} \left[\func[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}\right).
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
       & \mathbbm P\left( \mathbbm E_{\hyperpost} \left[\func[\expLossEnvRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}
        +
        \textup{B}_{\textup{e}}\right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%line 2
    & \leq
 \mathbbm P\Bigg( a_1\cdot \mathbbm E_{\hyperpost} \bigg[
 \func[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]}\nonumber\\
&\hspace{5em} +
 a_2\cdot\func[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}
 \bigg]\geq \textup{B}_{\textup{t}}
        +
        \textup{B}_{\textup{e}}\Bigg)\label{2021.02.21_22.38}\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%line 3
        &\leq
                  \mathbbm P\left(a_1\cdot \mathbbm E_{\hyperpost} \left[\func[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMeta[U]{\bm Z^\lenZm_i}{\task_i}}  \right]\geq 
        \textup{B}_{\textup{e}}\right)\nonumber\\
         &\hspace{5em}   +
                  \mathbbm P\left(a_2\cdot \mathbbm E_{\hyperpost} \left[\func[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}
\right),\label{2021.02.21_22.41}
\end{align}
where \eqref{2021.02.21_22.38} follows from
\eqref{2021.02.21_22.34}, and the fact that $\mathbbm P[A\geq a]\leq \mathbbm P[B\geq a]$ if $A\leq B$. Equation \ref{2021.02.21_22.41} is a direct result of \eqref{2021.02.21_23.12}, i.e.,
    \begin{align}
        \left\{(x_1,x_2):\;
        f_1(x_1)+f_2(x_2)\geq \textup{B}_\textup{t}+ \textup{B}_\textup{e}
        \right\}\subset
         \left\{x_1:\;
        f_1(x_1)\geq \textup{B}_\textup{t}
        \right\}\bigcup
              \left\{
        x_2:\;
        f_2(x_2)\geq \textup{B}_\textup{e}
        \right\}
    \end{align}
\end{proof}
\begin{corollary}
\label{cor1}
Under assumptions of Proposition \ref{prop-gen-pac-tsk} and \ref{prop-gen-pac-env}, for independent  tasks,
 with probability at least $1-\delta$ under $\mathrm P_{\trainEnv}$,  we have
 \begin{align}
      \mathbbm E_{\hyperpost} \left[
 \funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]}
 +
 \funcTsk[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}
 \right]\nonumber\\\leq \min_{\tau>1} \mathbbm E_{\hyperpost}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \textup{B}_{\textup{task}}\right]
        +
        \textup{B}_{\textup{env}},\label{cor1_first}
 \end{align}
 where
\begin{align}
 \textup{B}_\textup{task}= 
 \Dkl\left(\PWcondZimU||\PriorTsk  \right)
+\log\left(\frac{\tau\lenDataSet
\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta}\right),\label{b_tsk}
\end{align}
and
\begin{align}
     \textup{B}_\textup{env}=  \Dkl\left(\hyperpost||\PriorEnv  \right)
+\log\left(\frac{\tau
\mathbbm E_{\mathrm P_{\trainEnv}}\mathbbm E_{\PriorEnv}\, e^{\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}}}{(\tau-1)\delta}\right).\label{b_env}
\end{align}
 Additionally, consider the   case where in Proposition \ref{prop-gen-pac-tsk} and \ref{prop-gen-pac-env}, from   $\funcTsk[a]{b}\leq c_{\textup{tsk}}$ (res.  $\funcEnv[a]{b}\leq c_{\textup{env}}$), we can conclude 
$a\leq k_t\cdot b+ \funcinvTsk{c_{\textup{tsk}}}$ (resp. $a\leq k_e\cdot b+\funcinvEnv{c_{\textup{env}}}$) for $k_t\in\mathbbm R^+$ (resp. $k_e\in\mathbbm R^+$).
 Under this assumption, 
 with probability at least $1-\delta$ under $\mathrm P_{\trainEnv}$,  we have
  \begin{align}
      \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\expLossEnvRV\right]\leq  k_e\cdot k_t\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\empLossEnvRV
 \right] \hspace{7em}\nonumber\\+k_e\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet  \funcinvTsk{\textup{B}_{\textup{task}}}\right]
       +
       \funcinvEnv{ \textup{B}_{\textup{env}}}.\label{cor1_second}
 \end{align}
Finally,
let $\funcTsk[a]{b}=\funcEnv[a]{b}=\func[a]{b}$ denotes a measurable convex function satisfying \eqref{2021.02.21_22.34}. 
With probability at least $1-\delta$ under $\mathrm P_{\trainEnv}$, 
\begin{align}
    \mathbbm E_{\hyperpost} \left[\func[\expLossEnvRV]{\empLossEnvRV}  \right]\leq \min_{\tau>1}a_2\mathbbm E_{\hyperpost}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\textup{B}_{\textup{task}}\right]
        +
      a_1\textup{B}_{\textup{env}} ,\label{cor1_third}
\end{align}
where $a_1,a_2>0$ and are the coefficients in \eqref{2021.02.21_22.34}, 
 
\end{corollary}
\begin{proof}
 From Proposition \ref{prop-gen-pac-tsk}, for a given $u$, since we assume that the tasks are independent, by   averaging both sides of \eqref{prop-gen-pac-tsk_formula} over $\lenDataSet$, from Lemma \ref{Lemma_sum}, 
one can conclude that with probability at least $1-\sum_i\delta_i$ under $\mathrm P_{\trainTsk}$,  we have
\begin{align}
 \frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\funcTsk[\mathbbm E_{\PWcondZimU}(\expLossTskRV)]{\mathbbm E_{\PWcondZimU}(\empLossTskRV)}\hspace{10em}\nonumber\\
 \leq   
  \frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||\PriorTsk  \right)
+ \frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\log\left(\frac{
\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right).
\label{2021.03.10_10.39_b}
\end{align}
Note that \eqref{2021.03.10_10.39_b} is valid for any hyperparameter $u$. Averaging  both sides of \eqref{2021.03.10_10.39_b} over $\hyperpost$,  
with probability at least $1-\sum_i\delta_i$ under $\mathrm P_{\trainEnv}$,  we have
\begin{align}
\mathbbm E_{\hyperpost}\left[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \funcTsk[\mathbbm E_{\PWcondZimU}(\expLossTskRV)]{\mathbbm E_{\PWcondZimU}(\empLossTskRV)}\right]
 \leq \mathbbm E_{\hyperpost}\left[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet  \textup{B}_{\textup{task}}\right]
,\label{Pr-tsk0-a}
\end{align}
where the right hand side of \eqref{Pr-tsk0-a} is derived by setting  $\delta_i=\delta/(\tau.\lenDataSet) $.
Additionally, since $\funcTsk[]{}$ is convex, $\funcTsk[\frac{1}{\lenDataSet}\sum_i^{\lenDataSet} a_i]{\frac{1}{\lenDataSet}\sum_i^{\lenDataSet} b_i}\leq \frac{1}{\lenDataSet}\sum_i^{\lenDataSet}\funcTsk[a_i]{b_i}$, and hence  with probability at least $1-\sum_i\delta_i=1-\delta/\tau$ under $\mathrm P_{\trainEnv}$,  we have
\begin{align}
\mathbbm E_{\hyperpost}\left[
\funcTsk[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}\right]\label{Pr-tsk_a}\hspace{15em}\\
=\mathbbm E_{\hyperpost}\left[ \funcTsk[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \mathbbm E_{\PWcondZimU}(\expLossTskRV)]{\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\mathbbm E_{\PWcondZimU}(\empLossTskRV)}\right]\label{Pr-tsk_b}\\
\leq 
\mathbbm E_{\hyperpost}\left[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \funcTsk[\mathbbm E_{\PWcondZimU}(\expLossTskRV)]{\mathbbm E_{\PWcondZimU}(\empLossTskRV)}\right]\label{Pr-tsk_c}\\
 \leq  \mathbbm E_{\hyperpost}\left[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\textup{B}_{\textup{task}}\right],\label{Pr-tsk_d}
\end{align}
where in \eqref{Pr-tsk_b}, from Table \ref{table_notation},  we used the definition of meta-empirical loss and $\decomMetaRV$,  in  \eqref{Pr-tsk_c}, we applied the convexity of $\funcTsk[]{}$, and \eqref{Pr-tsk_d} follows from \eqref{Pr-tsk0-a}.

Next, by setting  
 $\delta_0=\frac{\tau-1}{\tau}\delta$ in \eqref{Pr_env}, we conclude that with probability at least $1-\frac{\tau-1}{\tau}\delta$, \eqref{Pr_env} holds.
Then in Lemma \ref{Lemma_sum}, by setting $\lenDataSet=2$, $a_1=\mathbbm E_{\hyperpost}1/\lenDataSet\sum_i \textup{B}_{\textup{task}}$,
 $a_2=\textup{B}_{\textup{env}}$, $f_1$ as the right hand side of \eqref{Pr-tsk_a}, and $f_2$ as the right hand side of \eqref{Pr_env}, we conclude \eqref{cor1_first}.

The proof of \eqref{cor1_second} is very similar. From \eqref{prop-gen-pac-tsk_formula}, with probability at least $1-\delta_i$ under $\mathrm P_{\trainTsk}$, we have 
\begin{align}
\mathbbm E_{\PWcondZimU}(\expLossTskRV)-\mathbbm E_{\PWcondZimU}(\empLossTskRV)%\hspace{15em}\nonumber\\
 \leq   
 \funcinvTsk{%\Dkl\left(\PWcondZimU||\PriorTsk  \right)
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right)
\Btsk}.
\label{2021.03.15_17.55}
\end{align}
Then, like before,  by   averaging both sides of \eqref{2021.03.15_17.55} over $\lenDataSet$ and over $\hyperpost$, from Lemma \ref{Lemma_sum}, 
%one can conclude that with probability at least $1-\sum_i\delta_i$ under $\mathrm P_{\trainEnv}$, 
%\begin{align}
%\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\mathbbm E_{\PWcondZimU}(\expLossTskRV)-\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\mathbbm E_{\PWcondZimU}(\empLossTskRV)\hspace{12em}\nonumber\\
% \leq   
% \frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\funcinvTsk{\Dkl\left(\PWcondZimU||\PriorTsk  \right)
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right)},
%\label{2021.03.15_17.55_a}
%\end{align}
%which is valid for any hyperparameter $u$. Averaging  both sides of \eqref{2021.03.15_17.55_a} over $\hyperpost$,  
with probability at least $1-\sum_i\delta_i$ under $\mathrm P_{\trainEnv}$,  we obtain
\begin{align}
\mathbbm E_{\hyperpost}\left[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\mathbbm E_{\PWcondZimU}(\expLossTskRV)-\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\mathbbm E_{\PWcondZimU}(\empLossTskRV)\right]\hspace{5em}\nonumber\\
 \leq   
\mathbbm E_{\hyperpost}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\funcinvTsk{%\Dkl\left(\PWcondZimU||\PriorTsk  \right)
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right)
\Btsk}\right].
\label{2021.03.15_17.55_b}
\end{align}
Similarly, from \eqref{Pr_env},  with probability at least $1-\delta_0$ under $\mathrm P_{\trainEnv}$, 
\begin{align}
\mathbbm E_{\hyperpost}\big(\expLossEnvRV\big)-\mathbbm E_{\hyperpost}\Big(\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV\Big)%\hspace{15em}\nonumber\\
 \leq   
\funcinvEnv{ %\Dkl\left(\hyperpost||\PriorEnv  \right)
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainEnv}}\mathbbm E_{\PriorEnv}\, e^{\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}}}{\delta_0}\right)
\Benv}.\label{2021.03.15_18.24}
\end{align}
Now, since $ \decomMeta[u]{\bm Z^\lenZm_i}{\task_i}=  \DefdecomMeta[u]{\bm Z^\lenZm_i}{\task_i}$,
 by setting $\lenDataSet=2$, $f_1$ the left hand side of \eqref{2021.03.15_17.55_b}, $f_2$ the left hand side of \eqref{2021.03.15_18.24}, and
$\mathbbm P_{X_i}=\mathrm P_{\trainEnv}$ , we find that with probability at least $1-\sum_i\delta_i-\delta_0$ under $\mathrm P_{\trainEnv}$
\begin{align}
\mathbbm E_{\hyperpost}\left[\expLossEnvRV\right]-\mathbbm E_{\hyperpost}\left[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\mathbbm E_{\PWcondZimU}(\empLossTskRV)\right]\hspace{10em}\nonumber\\
 \leq   
\funcinvEnv{ %\Dkl\left(\hyperpost||\PriorEnv  \right)
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainEnv}}\mathbbm E_{\PriorEnv}\, e^{\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}}}{\delta_0}\right)
\Benv}%\nonumber\\
+\mathbbm E_{\hyperpost}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\funcinvTsk{%\Dkl\left(\PWcondZimU||\PriorTsk  \right)
%+\log\left(\frac{
%\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right)
\Btsk}\right]
.\label{2021.03.15_18.31}
\end{align}
Finally, setting 
$\delta_0=\frac{\delta}{2}$, $\delta_i=\frac{\delta}{2\lenDataSet}$ in \eqref{2021.03.15_18.31}, we conclude \eqref{cor1_second}.

To prove  \eqref{cor1_third}, we note that since \eqref{2021.02.21_22.34} is satisfied,  we have
\begin{align}
    \mathbbm E_{\hyperpost} \left[ \func[\expLossEnvRV]{\empLossEnvRV}\right]\leq
    a_1 \mathbbm E_{\hyperpost} \left[\func[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}\right]\nonumber\\
    +a_2 \mathbbm E_{\hyperpost} \left[\func[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}\right]\nonumber
    \\
    \leq a_1 +a_2 \mathbbm E_{\hyperpost}\left[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\textup{B}_{\textup{task}}\right]
    \label{2021.03.17_17.09_b}
\end{align}
where  due to \eqref{Pr_env} and \eqref{Pr-tsk_d}.\eqref{2021.03.17_17.09_b} is valid with probability $1-\delta$. The proof is concluded by following the same approach. 
\end{proof}
\section{General Bound with Tuple Hypothesis Assumption}
\label{tuple-hypothesis}


To have a comprehensive setup, we provide the following proposition with the tuple hypothesis assumption. 
\begin{proposition}
\label{prop-gen-pac-tsk_two_KL}
Let $\funcTsk[a]{b}$ and $\funcEnv[a]{b}$ be functions which are convex in both $a$ and $b$. For any data-free or data-dependent prior $\PriorTsk$ and $\PriorEnv$, with probability at least $1-\delta$ under $\mathrm P_{\trainEnv}$,  we have
\begin{align}
\funcEnv[\mathbbm E_{\hyperpost}\left(
\expLossEnvRV
\right)]{\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)}\hspace{14em}\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
+\funcTsk[\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)]{\mathbbm E_{\hyperpost} \empLossEnvRV}\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \leq \min_{\theta_{\textup{tsk}},\theta_{\textup{env}}\geq 0}
 \log\frac{\mathbbm E_{\mathrm P_{\trainEnv}}\left(\Upsilon_{\textup{tsk}}^{\frac{1}{\theta_{\textup{tsk}}}}\cdot
     \Upsilon_{\textup{env}}^{\frac{1}{\theta_{\textup{env}}}}
\right)}{\delta}
+ \frac{1}{\theta_{\textup{tsk}}}
     \mathbbm E_{\hyperpost}\left(\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||
     \PriorTsk
     \right)\right)\nonumber\\
    + \left( \frac{1}{\theta_{\textup{tsk}}}+\frac{1}{\theta_{\textup{env}}}\right)\Dkl\left(\hyperpost||
     \PriorEnv
     \right),\label{cor_tup_1}
\end{align}
where
\begin{align}
\Upsilon_{\textup{env}}&=\mathbbm E_{\PriorEnv}e^{\theta_{\textup{env}}
\funcEnv[
\expLossEnvRV
]{\decomMetaRVTot}}\label{up_env}\\
\Upsilon_{\textup{tsk}}&=
     \mathbbm E_{ \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk} e^{ \theta_{\textup{tsk}}
     \funcTsk[%\frac{1}{\lenDataSet}\sum_{i=1}\lenDataSet
     \expLossTskRV]{%\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet
     \empLossTskRV}}\label{up_tsk}.
\end{align}

 %\begin{align}
 %     \mathbbm E_{\hyperpost} \left[
 %\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]}
 %+
 %\funcTsk[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}
 %\right]\nonumber\\\leq \mathbbm E_{\hyperpost}\left[ \Dkl\left( \hyperpost \prod_{i=1}^{\lenDataSet}\PWcondZimU\Big\|
  %   \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk \right)\right]
   %     +
%     \Dkl\left(\hyperpost||
%     \PriorEnv
 %    \right)\nonumber\\
 %   +  \log\frac{\mathbbm E_{\mathrm P_{\trainEnv}}\left(\Upsilon_{\textup{tsk}}\cdot
  %   \Upsilon_{\textup{env}}
%\right)}{\delta},\label{cor_tup_1}
% \end{align}
Additionally, for the case where  $\funcTsk[a]{b}=\funcTskRV(a-b)$ and  $\funcEnv[a]{b}=\funcEnvRV(a-b)$, and 
 $\funcinvTsk{\cdot}$ and  $\funcinvTsk{\cdot}$ denote the affine transform $\funcTskRV$ and $\funcEnvRV$, respectively, 
 with probability at least $1-\delta$ under $\mathrm P_{\trainEnv}$,  we have
       \begin{align}
\mathbbm E_{\mathrm P_{UW|\trainEnv}}\left(
\expLossEnvRV
\right)-\mathbbm E_{\hyperpost} \empLossEnvRV
    \hspace{20em}\nonumber\\
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
       \leq      %%%%%%%%%%%%%%%
     \funcinvEnv{\Dkl\left(\hyperpost||
     \PriorEnv
     \right)+
     \log\left(\frac{2
\mathbbm E_{\mathrm P_{ \trainEnv}}\Upsilon_{\textup{env}}}{\delta}\right)
     } 
     \hspace{10em}\nonumber\\
      +\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\funcinvTsk{
     \Dkl\left( \hyperpost \prod_{i=1}^{\lenDataSet}\PWcondZimU\Big\|
     \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk \right)
     +\log
      \frac{
2\lenDataSet\mathbbm E_{\mathrm P_{\trainEnv}}%\mathbbm E_{\PriorEnv\prod_i\PriorTsk}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta
\Upsilon_{\textup{tsk}}
}
%     \frac{2\mathbbm E_{\mathrm P_{\trainEnv}}\Upsilon_{\textup{tsk}}}
{\delta}}
,\label{cor_tup_2}
 \end{align}
 where $\Upsilon_{\textup{env}}$ and $\Upsilon_{\textup{tsk}}$ 
are given by \eqref{up_env} and \eqref{up_tsk}, respectively
 when $\theta_{\textup{tsk}}=
 \theta_{\textup{env}}=1$.
\end{proposition}
\begin{remark}
\label{rem1}
As mentioned before,  the advantage of assuming tuple-hypothesis is that the final expression 
in \eqref{cor_tup_1} has lower weights on the number of samples, i.e., $\log(\cdot/\delta)$.
This advantage comes from the fact that in the derivation of  \eqref{cor_tup_1},  Markov's inequality  was the final step (unlike Corollary \ref{cor1} which two Markov's inequality
ies are applied at both environment and task levels).
However, 
 \eqref{cor_tup_2} does not have the advantage of the tuple-hypothesis assumption, meaning that the we have both $\log(2(\cdot)/\delta)$ and $\log(2\lenDataSet(\cdot/)\delta)$ in  \eqref{cor_tup_2}. The reason is that to 
 obtain  \eqref{cor_tup_2} we applied two Markov's inequality. To be precise, since we assumed that   $\mathrm F^{\textup{Task}}$ is convex,  $\funcinvTsk{\cdot}$ is concave functions, and hence $\frac{1}{\lenDataSet}\sum_i \funcinvTsk{\cdot}\leq \funcinvTsk{\frac{1}{\lenDataSet}\sum_i\cdot}$. Thus, if we wanted to keep the advantage of  tuple-hypothesis assumption for  \eqref{cor_tup_2}, we would need to apply Markov's inequality after taking inverse function, and the final expression would have the term $\funcinvTsk{\frac{1}{\lenDataSet}\sum_i\cdot}$ which is looser than 
\eqref{cor_tup_1}, i.e.,  $\frac{1}{\lenDataSet}\sum_i \funcinvTsk{\cdot}$.
\end{remark}
\begin{proof}
 The steps are very similar to the proof of Corollary \ref{cor1}.
 At the task level, 
 by considering  $(u,w_1,...,w_\lenDataSet)$ as  a tuple of one prior and
$\lenDataSet$ base hypotheses, applying Jensen's inequality, and then  setting $\Posterior=\hyperpost \prod_{i=1}^{\lenDataSet}\PWcondZimU\triangleq\mathrm P_{UW|\trainEnv}$ as the posterior, $\Prior=\PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk$ as the prior, and $\funcTsk[]{}$ as $\phi$ in
 \eqref{Donsker}, we find that
 \begin{align}
 &\theta_{\textup{tsk}}\funcTsk[\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)]{\mathbbm E_{\hyperpost} \empLossEnvRV}
 \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\\
  &=\theta_{\textup{tsk}}\funcTsk[ \mathbbm E_{\mathrm P_{UW|\trainEnv}}\left(\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \expLossTskRV\right)]{ \mathbbm E_{\mathrm P_{UW|\trainEnv}}\left(\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\empLossTskRV\right)}  \\
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\textup{Jensen's inequality}\hspace{2em}   \leq
\mathbbm E_{\mathrm P_{UW|\trainEnv}} \left(\theta_{\textup{tsk}}\funcTsk[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \expLossTskRV]{\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\empLossTskRV}\right)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\ 
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%line2
  & \leq \Dkl\left(\mathrm P_{UW|\trainEnv}||
     \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk
     \right)  +\log\left(
     \mathbbm E_{ \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk}\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet e^{\theta_{\textup{tsk}}\funcTsk[ \expLossTskRV]{\empLossTskRV}}
     \right),
     \label{2021.03.10_15.13}
     \end{align}
     where in the above equations,  with some abuse of notation, we define $\mathrm P_{UW|\trainEnv}$
     as the product of two posteriors, i.e., $\hyperpost \prod_{i=1}^{\lenDataSet}\PWcondZimU$. 
 Applying this fact to the KL divergence term, and  using  $\log\prod_i a_i=\sum_i \log a_i$, we find that 
      \begin{align}
\funcTsk[\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)]{\mathbbm E_{\hyperpost} \empLossEnvRV}
      \leq
      \frac{1}{\theta_{\textup{tsk}}}
     \mathbbm E_{\hyperpost}\left(\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||
     \PriorTsk
     \right)\right)
     \nonumber\\
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
     +       \frac{1}{\theta_{\textup{tsk}}}\Dkl\left(\hyperpost||
     \PriorEnv
     \right)
     +\frac{1}{\theta_{\textup{tsk}}}\log\underbrace{\left(
     \mathbbm E_{ \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk} e^{ \theta_{\textup{tsk}} \funcTsk[%\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet
     \expLossTskRV]{%\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet
     \empLossTskRV}}
     \right)}_{\Upsilon_{\textup{tsk}}}.\label{2021.03.10_15.14}
 \end{align}

 

Similarly, at the environment level,
by marginalizing over $W$, using Jensen's inequality, and applying \eqref{Donsker},
we find that
\begin{align}
\theta_{\textup{env}}\funcEnv[\mathbbm E_{\mathrm P_{UW|\trainEnv}}\left(
\expLossEnvRV
\right)]{\mathbbm E_{\mathrm P_{UW|\trainEnv}}\left(\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet  \decomMetaRV\right)}\hspace{5em }\nonumber\\
=\theta_{\textup{env}}\funcEnv[\mathbbm E_{\hyperpost}\left(
\expLossEnvRV
\right)]{\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)}\\
\leq
\Dkl\left(\hyperpost||
     \PriorEnv
     \right)+\log\underbrace{\left(\mathbbm E_{\PriorEnv}e^{\theta_{\textup{env}}\funcEnv[
\expLossEnvRV
]{\decomMetaRVTot}}\right)}_{\Upsilon_{\textup{env}}}.\label{2021.03.10_15.15}
\end{align}

Now, summing both sides of \eqref{2021.03.10_15.13} and \eqref{2021.03.10_15.15}, in view of \eqref{2021.03.10_15.14}, and using the fact that $\log(a)+\log(b)=\log(a.b)$, we finally obtain
\begin{align}
\func[\mathbbm E_{\hyperpost}\left(
\expLossEnvRV
\right)]{\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)}\hspace{10em}\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
+\func[\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)]{\mathbbm E_{\hyperpost} \empLossEnvRV}\leq \log\left(\Upsilon_{\textup{tsk}}^{\frac{1}{\theta_{\textup{tsk}}}}\cdot
     \Upsilon_{\textup{env}}^{\frac{1}{\theta_{\textup{env}}}}
\right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
+ \frac{1}{\theta_{\textup{tsk}}}
     \mathbbm E_{\hyperpost}\left(\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||
     \PriorTsk
     \right)\right)
%\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
+\left( \frac{1}{\theta_{\textup{tsk}}}+\frac{1}{\theta_{\textup{env}}}\right)\Dkl\left(\hyperpost||
     \PriorEnv
     \right)
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %   +\log\left(\mathbbm E_{\PriorEnv}e^{\theta_{\textup{env}}\func[
%\expLossEnvRV
%]{\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \expLossTskRV}}\right)^{\frac{1}{\theta_{\textup{env}}}}\cdot
%\left(
%     \mathbbm E_{ \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk} e^{ \theta_{\textup{tsk}} \func[\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \expLossTskRV]{\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\empLossTskRV}}
 %    \right)^{\frac{1}{\theta_{\textup{tsk}}}},
 \\
 \leq
 \log\frac{\mathbbm E_{\mathrm P_{\trainEnv}}\left(\Upsilon_{\textup{tsk}}^{\frac{1}{\theta_{\textup{tsk}}}}\cdot
     \Upsilon_{\textup{env}}^{\frac{1}{\theta_{\textup{env}}}}
\right)}{\delta}+ \frac{1}{\theta_{\textup{tsk}}}
     \mathbbm E_{\hyperpost}\left(\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||
     \PriorTsk
     \right)\right)\nonumber\\
    + \left( \frac{1}{\theta_{\textup{tsk}}}+\frac{1}{\theta_{\textup{env}}}\right)\Dkl\left(\hyperpost||
     \PriorEnv
     \right)
 ,
\end{align}
where in the last step, we applied Markov's inequality. By optimization over $\theta_{\textup{tsk}}$ and $\theta_{\textup{env}}$, we conclude the proof. 



Next, to prove \eqref{cor_tup_2}, we follow exactly the same steps presented in the proof of \eqref{cor1_second}, by replacing  $\PWcondZimU$ and $\PriorTsk$ with $\hyperpost \prod_{i=1}^{\lenDataSet}\PWcondZimU$ and 
$\PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk$, respectively.



%by applying Markov's inequality to \eqref{2021.03.10_15.14} and setting $\theta_{\textup{tsk}}=1$, with probability at least $1-\delta_i$ under probability $\mathrm P_{\trainEnv}$, we have
%    \begin{align}
%\funcTsk[\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)]{\mathbbm E_{\hyperpost} \empLossEnvRV}
 %   \hspace{15em} \nonumber\\  \leq
 %    \mathbbm E_{\hyperpost}\left(\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||
  %   \PriorTsk
   %  \right)\right)
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % +      \Dkl\left(\hyperpost||
   %  \PriorEnv
%     \right)
 %    +\log\frac{\mathbbm E_{\mathrm P_{\trainEnv}}\Upsilon_{\textup{tsk}}}{\delta_i}.\label{2021.03.10_15.14_b}
 %\end{align}
%Now,
 %considering the fact that $\funcTsk[a]{b}=\funcTskRV(a-b)$ and in view of $\funcinvTsk{}$, from \eqref{2021.03.10_15.14_b}, we find that 
 %     \begin{align}
%\mathbbm E_{\hyperpost}\left( \decomMetaRVTot\right)-\mathbbm E_{\hyperpost} \empLossEnvRV
 %    \hspace{17em}\nonumber\\
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %     \leq
%      \funcinvTsk{
   %  \mathbbm E_{\hyperpost}\left(\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||
 %    \PriorTsk
  %   \right)\right) +  \Dkl\left(\hyperpost||
   %  \PriorEnv
%     \right)
%     +\log\frac{\mathbbm E_{\mathrm P_{\trainEnv}}\Upsilon_{\textup{tsk}}}{\delta_i}}.\label{2021.03.10_15.15_a}
 %\end{align}
 % Averaging both sides of \eqref{2021.03.10_15.15_a} over $\lenDataSet$
 
 %
 %Similarly by applying Markov's inequality to \eqref{2021.03.10_15.15}, and setting $\theta_{\textup{env}}=1$ and  $\funcEnv[a]{b}=\funcEnvRV(a-b)$,  with probability at least $1-\delta_e$ under probability $\mathrm P_{\trainEnv}$,  we find that
 %\begin{align}
%\mathbbm E_{\mathrm P_{UW|\trainEnv}}\left(
%\expLossEnvRV
%\right)-\mathbbm E_{\mathrm P_{UW|\trainEnv}}\left(\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet  \decomMetaRV\right)\hspace{5em }\nonumber\\
%\leq
%\funcinvEnv{\Dkl\left(\hyperpost||
 %    \PriorEnv
  %   \right)+\log\frac{\mathbbm E_{\mathrm P_{\trainEnv}}\Upsilon_{\textup{env}}}{\delta_e}}.\label{2021.03.10_15.15_b}
%\end{align}
%Summing both sides of \eqref{2021.03.10_15.15_a} and \eqref{2021.03.10_15.15_b},setting $\delta_t=\delta_e=0.5\delta$ from Lemma \ref{Lemma_sum}, we conclude \eqref{cor_tup_2}.
\end{proof}

\section{Re-obtaining Existing Results}
\label{pre_works}
Here, to the best of my knowledge, we present  
the main PAC-Bayes bounds for the meta-learning problem. 

Firstly,  to obtain \eqref{amit_th2}, 
we set $\funcTsk[a]{b}=2(\lenZm_i-1)(a-b)^2$, $\funcEnv[a]{b}=2(\lenDataSet-1)(a-b)^2$ in \eqref{cor_tup_2}.These choices lead to $\funcinvTsk{a}=\sqrt{\frac{a}{2(\lenZm_i-1)}}$ and also  $\funcinvEnv{a}=\sqrt{\frac{a}{2(\lenDataSet-1)}}$. To bound 
$\mathbbm E[\Upsilon_{\textup{env}}]$ and 
$\mathbbm E[\Upsilon_{\textup{tsk}}]$, in view of Lemma \ref{prior-indep},  
we set $\PriorTsk=\mathrm P_{W|U}$ and $\PriorEnv=\hyperprior$.  Since the prior in independent of the data, by interchanging the order of expectations over $\mathrm P_{ \trainEnv}$ and priors, we find that
\begin{align}
 &   \mathbbm E_{\mathrm P_{ \trainEnv}}\left[  \Upsilon_{\textup{env}}\right]=
    \mathbbm E_{\PriorEnv}  \mathbbm E_{\mathrm P_{ \trainEnv}}\left[  e^{
2(\lenDataSet-1)\left(
\expLossEnvRV
-\decomMetaRVTot\right)^2}\right]  \leq \lenDataSet,\label{2021.03.21_08.25}\\
%%%%%%%%%%%%%%%%
  &  \mathbbm E_{\mathrm P_{ \trainEnv}}\left[  \Upsilon_{\textup{tsk}}\right]=
        \mathbbm E_{ \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk}  \mathbbm E_{\mathrm P_{ \trainEnv}}\left[  e^{
2(\lenZm_i-1)\left(
 \expLossTskRV-  \empLossTskRV\right)^2}\right]  \leq \lenZm_i,\label{2021.03.21_08.26}
\end{align}
where in \eqref{2021.03.21_08.25},  we used Lemma \ref{prior-indep} by setting  $\lambda=\frac{2(\lenDataSet-1)}{\lenDataSet}$ and $\sigma=0.5$, and in \eqref{2021.03.21_08.26} we set $\lambda=\frac{2(\lenZm_i-1)}{\lenZm_i}$ and $\sigma=0.5$. We recall that 
since the loss function is bounded on $[0,1]$, we set $\sigma=0.5$ in Lemma \ref{prior-indep}. Now, applying these facts to \eqref{cor_tup_2}, we find that
       \begin{align}
\mathbbm E_{\hyperpost}\left(
\expLossEnvRV
\right)-\mathbbm E_{\hyperpost} \empLossEnvRV
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
       \leq      %%%%%%%%%%%%%%%
     \sqrt{\frac{\Dkl\left(\hyperpost||
     \PriorEnv
     \right)+
     \log\left(\frac{2
\lenDataSet}{\delta}\right)
    }{2(\lenDataSet-1)} } 
     \hspace{0em}\nonumber\\
      +\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\sqrt{\frac{
     \Dkl\left( \hyperpost \prod_{i=1}^{\lenDataSet}\PWcondZimU\Big\|
     \PriorEnv\prod_{i=1}^{\lenDataSet}\PriorTsk \right)
     +\log
      \frac{
2\lenDataSet\lenZm_i
}
{\delta}}{2(\lenZm_i-1)}},
 \end{align}
 which is the same is \eqref{amit_th2}.

Now, to obtain \eqref{rothfuss_th2}, in \eqref{cor_tup_1} we set $\funcEnv[a]{b}=\funcTsk[a]{b}=(a-b)$,  $\theta_{\textup{tsk}}=\beta$, and $\theta_{\textup{env}}=\lambda$, and then 
\begin{align}
\mathbbm E_{\hyperpost}\left(
\expLossEnvRV
\right)-\mathbbm E_{\hyperpost} \empLossEnvRV
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \leq \min_{\beta,\lambda\geq 0}
(\frac{\lambda}{8\lenDataSet}+\frac{\lambda}{8\lenZm})-\frac{1}{\sqrt\lenDataSet}\log\delta
\nonumber\\
+ \frac{1}{\beta}
     \mathbbm E_{\hyperpost}\left(\sum_{i=1}^{\lenDataSet}\Dkl\left(\PWcondZimU||
     \PriorTsk
     \right)\right) 
    + \left( \frac{1}{\beta}+\frac{1}{\lambda}\right)\Dkl\left(\hyperpost||
     \PriorEnv
     \right),
\end{align}
which is the same as \eqref{rothfuss_th2}.



Finally, to obtain \eqref{Implicit_Prior_Th1}, 
we set $\funcTsk[a]{b}=2(\lenZm_i-1)(a-b)^2$, $\funcEnv[a]{b}=2(\lenDataSet-1)(a-b)^2$ in \eqref{cor1_second}. These choices lead to $\funcinvTsk{a}=\sqrt{\frac{a}{2(\lenZm_i-1)}}$ and also  $\funcinvEnv{a}=\sqrt{\frac{a}{2(\lenDataSet-1)}}$. Setting $\PriorTsk=\mathrm P_{W|U}$ and $\PriorEnv=\hyperprior$ in  Corollary \ref{cor1}, since $\PriorTsk$ (resp. $\PriorEnv$) is independent of data, we can exchange the order of expectations over $\mathrm P_{\trainTsk}$ (resp. $\mathrm P_{\trainEnv}$) with $\PriorTsk$ (resp. $\PriorEnv$) in \eqref{b_tsk} (resp. \eqref{b_env}). Applying Lemma  \ref{prior-indep}, in view of \eqref{2021.03.21_08.25} and \eqref{2021.03.21_08.26}, we find that
\begin{align}
    \mathbbm E_{\hyperpost} \left[\expLossEnvRV-\empLossEnvRV
 \right]\leq
    \sqrt{\frac{\Dkl\left(\hyperpost||\PriorEnv  \right)
+  \log\left(\frac{2
\lenDataSet}{\delta}\right)}{2(\lenDataSet-1)}}
 \nonumber\\+
 \mathbbm E_{\hyperpost}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet  
 \sqrt{\frac{\Dkl\left(\PWcondZimU||\PriorTsk  \right)+\log\left(\frac{2\lenDataSet
\lenZm_i}{\delta}\right)}{2(\lenZm_i-1)}}
 \right].\label{gom1}
\end{align}
Since $\sqrt{a}$ is a concave function, we have $\sqrt{\mathbbm E[X]}\geq \mathbbm E[\sqrt X]$. By taking the expectation over $\hyperpost$ inside the radical of the last term in \eqref{gom1}, it can be verified that  
\eqref{gom1} is upper bounded by
\begin{align}
       \mathbbm E_{\hyperpost} \left[\expLossEnvRV-\empLossEnvRV
 \right]\leq
    \sqrt{\frac{\Dkl\left(\hyperpost||\PriorEnv  \right)
+  \log\left(\frac{2
\lenDataSet}{\delta}\right)}{2(\lenDataSet-1)}}
 \nonumber\\+
  \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet  
 \sqrt{\frac{\mathbbm E_{\hyperpost}\left[\Dkl\left(\PWcondZimU||\PriorTsk  \right)\right]+\log\left(\frac{2\lenDataSet
\lenZm_i}{\delta}\right)}{2(\lenZm_i-1)}  }
\end{align}
which is tighter than both \eqref{amit_th2} and \eqref{Implicit_Prior_Th1}. 

\section{New PAC-Bayes Bounds for Meta learning}
\label{our-bounds}
In this section, in view of Corollary \ref{cor1}, we obtain new bounds for the meta-generalization error. We use \eqref{cor1_first} to find bounds.
\begin{itemize}
    \item The loss function is bounded by  $\mathrm L_{\max}$; $\funcEnv[a]{b}=\lenDataSet\Dkl(a,b)$ and $\funcTsk[a]{b}=\lenZm\Dkl(a,b)$ (all $\lenZm_i=\lenZm$ or $\lenZm=\max M_i$):
     \begin{align}
      \lenDataSet\mathbbm E_{\hyperpost} \left[
 \lenDataSet\Dkl\left(\frac{\expLossEnvRV}{\mathrm L_{\max}}\big\|\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet} \frac{\decomMetaRV}{\mathrm L_{\max}}   ]\right)
 +
  \lenZm\Dkl\left(\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \frac{\decomMetaRV}{\mathrm L_{\max}}\Big\|\frac{\empLossEnvRV}{\mathrm L_{\max}}\right)
 \right]\nonumber\\\leq \min_{\tau>1} \mathbbm E_{\hyperpost}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \Dkl\left(\PWcondZimU||\PriorTsk  \right)
+\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\log\left(\frac{2\tau\lenDataSet\sqrt{\lenZm_i}
}{\delta}\right)\right]
  \nonumber\\      +
\Dkl\left(\hyperpost||\PriorEnv  \right)
+\log\left(\frac{2\tau\sqrt{\lenDataSet}
}{(\tau-1)\delta}\right),\label{2021.03.21_10.53}
 \end{align}
 where in \eqref{2021.03.21_10.53}, we used Lemma \ref{kl_lem}.
 
 \item 
 Combining the facts that  $\Dkl(a||b)\geq 2(a-b)^2$ and  $\frac{2\lenDataSet\lenZm}{\lenDataSet+\lenZm}(a-c)^2\leq 2\lenDataSet(a-b)^2+ 2\lenZm(b-c)^2$, we conclude 
 $\frac{2\lenDataSet\lenZm}{\lenDataSet+\lenZm}(a-c)^2\leq \lenDataSet \Dkl(a||b)+\lenZm\Dkl(b||c)$. 
 Inserting this inequality to \eqref{2021.03.21_10.53}, and  recalling  that $(\mathbbm E [A-C])^2\leq \mathbbm E [A-C]^2$, we find that
 \begin{align}
    \left |\mathbbm E_{\hyperpost} \left[
   \expLossEnvRV- \empLossEnvRV \right] \right|
   \leq \min_{\tau>1}\mathrm L_{\max}\frac{\lenDataSet+\lenZm}{2\lenDataSet\lenZm}\Bigg(\Dkl\left(\hyperpost||\PriorEnv  \right)
\hspace{5em}\nonumber\\
%%%%%%%%%%
+\log\left(\frac{2\tau\sqrt{\lenDataSet}
}{(\tau-1)\delta}\right)
+\mathbbm E_{\hyperpost}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \Dkl\left(\PWcondZimU||\PriorTsk  \right)
+\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\log\left(\frac{2\tau\lenDataSet\sqrt{\lenZm_i}
}{\delta}\right)\right]
\Bigg)^\frac{1}{2}
 \end{align}
 
 \item Fast rate: 
 \begin{align}
   \mathbbm E_{\hyperpost} \left[
   \expLossEnvRV\right]\leq
   \min_{\lambda_e,\lambda_t\geq 0.5}
      \frac{1}{1-\frac{1}{2\lambda_e}}\cdot \frac{\mathbbm E_{\hyperpost}\empLossEnvRV}{1-\frac{1}{2\lambda_t}}+
 \frac{\log(\frac{2}{\delta})}{{1-\frac{1}{2\lambda_e}}} \left(\lambda_e+ \frac{\lambda_t }{1-\frac{1}{2\lambda_t}}
 \right)\nonumber\\
      \frac{\lambda_e}{1-\frac{1}{2\lambda_e}}\left(
   \Dkl\left( \hyperpost \Big\|   \PriorEnv\right) \right)+ 
       \frac{1}{1-\frac{1}{2\lambda_e}}\cdot \frac{\lambda_t}{1-\frac{1}{2\lambda_t}}\left( 
       \Dkl\left(\mathrm P_{UW|\trainEnv}
       \Big\| \mathrm P_{UW}
       \right)
    \right)
 \end{align}
 
\item  Set $\func[a]{b}=|a-b|$,
    $\theta_{task}=\sqrt{\lenZm}$, $\theta_{\textup{env}}=\sqrt{\lenDataSet}$,  $\PriorTsk\propto e^{\gamma_{\textup{task}}\empLossTskRV}$, $\PriorEnv\propto e^{\gamma_{\textup{env}}\empLossEnvRV}$,          \begin{align}
       \expLossEnvRV-\empLossEnvRV\leq \min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} 
        \frac{1}{\sqrt{\lenDataSet}}\Dkl\left(\hyperpost||\PriorDataDepEnv[U]{\trainEnv}{} \right)\nonumber\\
     +\mathbbm E_{\hyperpost}\frac{1}{\lenDataSet\cdot\sqrt{\lenZm}}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimU||\PriorDataDepTsk[W]{\trainTsk}{U}  \right)\right]\nonumber\\
     +\frac{2(1+\frac{2\gamma_{\textup{task}}}{\sqrt{\lenZm}})+ \log\frac{2\lenDataSet(1+\sqrt{e})}{\delta}}{\sqrt{\lenZm}}
     +\frac{2(1+\frac{2\gamma_{\textup{env}}}{\sqrt{\lenDataSet}})+ \log\frac{2(1+\sqrt{e})}{\delta}}{\sqrt{\lenDataSet}}.
        \end{align}     
\end{itemize}

\section{Numerical Results}
\label{num_res}
To compare the results, we set

\section{General Lemmas}
\label{gen_lemma}
In this section, we provide a number of general lemmas that will be used through the paper.
\begin{lemma}
\label{prior-indep}
Let $X_1,...,X_m$ be i.i.d. random variables. Assume $\Delta=\mathbbm E[g(X)]-\frac{1}{m}\sum_{k=1}^mg(X_i)$.
If for $\epsilon>0$, we have $\mathbbm P[\Delta\geq \epsilon ]\leq \exp(\frac{-m\epsilon^2}{2\sigma^2})$, then 
\begin{align}
    \mathbbm E\left[e^{\lambda m \Delta^2}  \right]\leq \frac{1}{1-2\lambda\sigma^2}, 
\end{align}
for $\lambda\leq\frac{1}{2\sigma^2}$.
\end{lemma}
\begin{proof}
The proof is similar to \cite[Lemma 3]{McAllaster1999}. For completeness, we repeat it again. 
Let $f^\star$ denotes the density function maximizing $\mathbbm E[e^{\lambda m \Delta^2} ]$ subject to the constraint that $\mathbbm P[\Delta\geq \epsilon ]\leq \exp(\frac{-m\epsilon^2}{2\sigma^2})$. The maximum occurs when $\mathbbm P_{f^\star}[\Delta\geq \epsilon ]= \exp(\frac{-m\epsilon^2}{2\sigma^2})$ leading to
\begin{align}
  f^\star(\Delta)=\frac{m\Delta}{\sigma^2} \exp\left( -\frac{m\Delta^2}{2\sigma^2} \right)\mathbbm{1} \{ \Delta\geq 0 \}.
\end{align}
Thus, we have
\begin{align}
      \mathbbm E\left[e^{\lambda m \Delta^2}  \right]\leq \int_{0}^{\infty}  \exp\left(\lambda m \Delta^2\right)\frac{m\Delta}{\sigma^2} \exp\left( -\frac{m\Delta^2}{2\sigma^2} \right) d\Delta =\frac{1}{1-2\lambda\sigma^2},\hspace{2em} \lambda<\frac{1}{2\sigma^2}.
\end{align}
\end{proof}



\begin{lemma}
\label{prior-indep-square}
Let $X_1,...,X_m$ be i.i.d. random variables. Assume $\Delta=\mathbbm E[g(X)]-\frac{1}{m}\sum_{k=1}^mg(X_i)$, where $g(\cdot)$ is sub-Gaussian with parameter $\sigma$. 
Then ,
\begin{align}
    \mathbbm E\left[e^{\lambda m \Delta^2}  \right]\leq \frac{1}{\sqrt{1-2\lambda\sigma^2}}, 
\end{align}
for $\lambda\leq\frac{1}{2\sigma^2}$.
\end{lemma}
\begin{proof}
The proof is similar to \cite[Th. 2.6]{Wainwright}. For completeness, we repeat it again.
Since $g(\cdot)$ is sub-Gaussian, we have
\begin{align}
    \mathbbm E\left[ e^{\lambda\Delta} \right]\leq \exp\left( \frac{\lambda^2\sigma^2}{2m} \right).\label{201.03.16_14.27}
\end{align}
Multiplying both sides of \eqref{201.03.16_14.27} by $\exp(-\frac{\lambda^2\sigma^2}{2sm})$ for $s\in(0,1)$, we find that
\begin{align}
    \mathbbm E\left[ e^{\lambda\Delta-\frac{\lambda^2\sigma^2}{2sm}} \right]\leq \exp\left( \frac{-\lambda^2\sigma^2}{2ms}(-s+1) \right).\label{201.03.16_14.29}
\end{align}
Next, we take integration with respect to $\lambda$. 
Since \eqref{201.03.16_14.29} is valid for any $\lambda\in\mathbbm R$, by using Fubini's theorem, we exchange the order of expectation and integration, leading to
\begin{align}
    \mathbbm E\left[ \exp\left(\frac{s m\Delta^2}{2\sigma^2}\right) \right]\leq \frac{1}{\sqrt{1-s}},\hspace{2em}\textup{for }0<s<1.
\end{align}
By defining $\lambda=\frac{s}{2\sigma^2}$, we conclude the proof.
\end{proof}


\begin{lemma}
\label{kl_lem}
Let $X_1,...,X_n$ be i.i.d random variables, and   $f:\mathcal X\rightarrow[0,1]$ be a bounded function. For all $n>8$, we have
\begin{align}
    \mathbbm E\left[e^{\Dkl\left( \frac{1}{n}\sum_i f(X_i)|| \mathbbm E[f(X)]  \right) } \right] \leq 2\sqrt{n}.
    \end{align}
\end{lemma}
\begin{proof}
 See \cite[Th. 1]{Maurer}, then for $n\geq 8$, the right hand side of \cite[Eq. (5)]{Maurer} is smaller than $\sqrt{n}$.
\end{proof}


\begin{lemma}
\label{D_gama}
Let $X_1,...,X_n$ be i.i.d random variables. For the given function  $f:\mathcal X\rightarrow[0,1]$, we have
\begin{align}
    \mathbbm E\left[e^{n\Dgama\left(\frac{1}{n}\sum_i f(X_i) ||\mathbbm E[f(X)] \right)}  \right]\leq 1.
\end{align}
\end{lemma}
\begin{proof}
 See \cite[Eq. 18]{McAllester2013}.  For completeness, we repeat it again. Since for $a\in[0,1]$ and $\gamma\in\mathbbm R$, we have $e^{\gamma a}\leq 1-a+a\cdot e^\gamma$, we conclude $   e^{\frac{\gamma}{n}\sum_i f(X_i) }\leq 1-\frac{1}{n}\sum_i f(X_i)+e^\gamma  \frac{1}{n}\sum_i f(X_i) $, by taking expectation from both sides, we find that $\mathbbm E\left[e^{\frac{\gamma}{n}\sum_i f(X_i) }\right]\leq 1-\mathbbm E\left[ f(X) \right]+e^\gamma  \mathbbm E\left[ f(X) \right]$. Taking logarithm from both sides leads to
 \begin{align}
\mathbbm E\left[e^{\frac{\gamma}{n}\sum_i f(X_i) -\log\left( 1-\mathbbm E\left[ f(X) \right]+e^\gamma  \mathbbm E\left[ f(X) \right]\right)}\right]\leq 1 \label{2021.03.19_.8.47}
 \end{align}
 Now, since $X_i$s are independent
 \begin{align}
     \mathbbm E_{\mathrm P_{\bm X_{1:n}}}\Big [& e^{n\Dgama\left(\frac{1}{n}\sum_i f(X_i) ||\mathbbm E[f(X)] \right)}  \Big]=
          \mathbbm E_{\mathrm P_{\bm X_{1:n}}}\left [ \prod_{i=1}^n e^{\Dgama\left(\frac{1}{n}\sum_i f(X_i) ||\mathbbm E[f(X)] \right)}  \right]
          %%%%%%%%%%%%
          \\
          &=\prod_{i=1}^n \mathbbm E_{\mathrm P_{X_i}}\left [  e^{\Dgama\left(\frac{1}{n}\sum_i f(X_i) ||\mathbbm E[f(X)] \right)}  \right]
          %%%%%%%%%%
          \\
\textup{Definition of } \Dgama\hspace{1em}          &=\prod_{i=1}^n \mathbbm E_{\mathrm P_{X_i}}\left [  e^{\frac{\gamma}{n}\sum_i f(X_i) -\log(1-\mathbbm E[f(X)]+e^\gamma  \mathbbm E[f(X)])}  \right]\underbrace{\leq}_{ \eqref{2021.03.19_.8.47}} 1.
 \end{align}
\end{proof}

\begin{lemma}
\label{Arezou_Bnd}
Let $\phi(\cdot)$ be a measurable  function which is bounded on the interval $[\phi_{\min},\phi_{\max}]$ for all $x\in\mathcal R$. For any two distributions $\Prior,\Posterior\in\mathcal P_{\mathcal X}$, we have
\begin{align}
     \mathbbm E_{\Posterior} [\phi]\leq \min_{\alpha\in[0,1]} \mathrm D_{\textup{KL}}(\Posterior||\Prior)-\DAre[\alpha]{\Posterior}{\Prior}+\log\left(
        \mathbbm E_{\Prior} \left[e^{\phi}\right]
        \right),\label{newOne}
\end{align}
where
\begin{align}
  \DAre[\alpha]{\Posterior}{\Prior}=\frac{1}{2}\Big((1-\alpha)\mathbbm P_{\Posterior}\left[ \alpha \Posterior(X)\geq \Prior(X)e^{\phi_{\max}-\phi_{\min}}\right]  \Big)^2
  \\
    =
  \frac{1}{2}\left(\sum_{\substack{x:\\\alpha\Posterior(x)\geq \Prior(x)\cdot e^{\phi_{\max}-\phi_{\min}}|_{\alpha\in(0,1)}}}(1-\alpha)\Posterior(x) \right)^2.
\end{align}
\end{lemma}
\begin{proof}
 For any $\alpha\in[0,1]$
    \begin{align}
       \mathbbm E_{\Posterior} [\phi]-
               \log\left(\mathbbm E_{\Prior} \left[e^{\phi}\right]\right)&=
               \sum_x \Posterior(x)\phi(x)
               -
               \log\left(\sum_x\Prior(x) e^{\phi(x)}\right)
               \\
               %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     =\sum_x\Posterior(x)\log\Big(&\frac{e^{\phi(x)}}{\sum_{\bar x}\Prior(\bar x) e^{\phi(\bar x)}}\Big)
               \\
               %%%%%%%%%%%%%%%%%%line 2
               =\sum_x \Posterior(x)\log\Big(
              \frac{\Posterior(x)}{\Posterior(x)}& \cdot\frac{\Prior(x)e^{\phi(x)}}{\Prior(x)\sum_{\bar x}\Prior(\bar x) e^{\phi(\bar x)}}
               \Big)=
               \sum_x \Posterior(x)\log\left(
\frac{\Posterior(x)}{\Posterior(x)}\cdot
\frac{\tildePrior(x)}{\Prior(x)}
               \right)\label{2020.02.08_10.41}
               \\
               %%%%%%%%%%%%%%%%%%%%%%%%%line 3
               &=\mathrm D_{\textup{KL}}(\Posterior||\Prior)-\underbrace{\mathrm D_{\textup{KL}}(\Posterior||\tildePrior)}_{\textup{For Donsker:} \geq 0}\label{2020.02.08_10.42}\\
               %%%%%%%%%%%%%%%%%%%%%%%%%%%%line 4
             \textup{Pinsker’s inequality}  \hspace{3em} &\leq
               \mathrm D_{\textup{KL}}(\Posterior||\Prior)-\frac{1}{2}\left(
               \sum_x \left|
               \Posterior(x)-\tildePrior(x)
               \right|
               \right)^2\label{2020.02.08_10.49}
               \end{align}
    \begin{align}  
            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%line 5
            =
                  \mathrm D_{\textup{KL}}(\Posterior||\Prior)-&\frac{1}{2}\left(
               \sum_{x: \alpha \Posterior(x)\geq \tildePrior(x)} 
                \underbrace{ 
               \left(
              \Posterior(x)-\tildePrior(x)\right)}_{\geq (1-\alpha)\Posterior(x)}
               +
                        \underbrace{      \sum_{x:\alpha \Posterior(x)< \tildePrior(x)} \left|
               \Posterior(x)-\tildePrior(x)
               \right|}_{\geq 0}
               \right)^2\label{2020.02.08_10.50}\\
               %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% line 6
              & \leq 
                \mathrm D_{\textup{KL}}(\Posterior||\Prior)-\frac{1}{2}\left(
               \sum_{x: \alpha \Posterior(x)\geq \tildePrior(x)}              (1-\alpha)\Posterior(x)
               \right)^2\\
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\line 7
                & \leq 
                \mathrm D_{\textup{KL}}(\Posterior||\Prior)-\frac{1}{2}\left(
               \sum_{x: \alpha\Posterior(x)\geq \Prior(x)\cdot e^{\phi_{\max}-\phi_{\min}}}              (1-\alpha)\Posterior(x)
               \right)^2,\label{2020.02.08_10.57}
    \end{align}
    where in \eqref{2020.02.08_10.41}, we define
    \begin{align}
        \tildePrior(x)=\frac{\Prior(x)e^{\phi(x)}}{\sum_{\bar x}\Prior(\bar x) e^{\phi(\bar x)}}.
    \end{align}
    Equation \eqref{2020.02.08_10.49} follows from Pinsker’s inequality in the form of
    \begin{align}
        \mathrm D_\textup{KL}(\Posterior||\tildePrior)\geq \frac{1}{2}\| \Posterior-\tildePrior\|_1^2\geq \frac{1}{2}\left(
               \sum_x \left|
               \Posterior(x)-\tildePrior(x)
               \right|
               \right)^2.
    \end{align}
    Finally, in \eqref{2020.02.08_10.57}, we used the fact that
    \begin{align}
              \underbrace{  \left\{x: \alpha\Posterior(x)\geq \Prior(x)\cdot e^{\phi_{\max}-\phi_{\min}}\right\}   }_{\mathcal A} \subseteq 
                               \underbrace{ \left\{x: \alpha\Posterior(x)\geq \frac{\Prior(x)e^{\phi(x)}}{\sum_{\bar x}\Prior(\bar x) e^{\phi(\bar x)}}\right\}}_{\mathcal B}. \label{2021.02.08_11.23}
    \end{align}
    To show \eqref{2021.02.08_11.23}, i.e., to show $\mathcal A\subset \mathcal B$, we prove that if $x\notin\mathcal B$ then $x\notin\mathcal A$. Assume $x\notin \mathcal B$, then 
    \begin{align}
        \alpha\Posterior(x)<
               \frac{\Prior(x) e^{\phi(x)}} {\sum_{\bar x}\Prior(\bar x) e^{\phi(\bar x)}}, \;\Rightarrow \;
                \alpha\Posterior(x)<
                             \frac{\Prior(x) e^{\phi_{\max}}} {\sum_{\bar x}\Prior(\bar x) e^{\phi(\bar x)}}\leq
                             \frac{\Prior(x) e^{\phi_{\max}}} {\sum_{\bar x}\Prior(\bar x) e^{\phi_{\min}}}\leq  \Prior(x)\cdot e^{\phi_{\max}-\phi_{\min}},
               \end{align}
   where  the last inequality means $x\notin\mathcal A$.
  Since  from  $x\notin\mathcal B$, then  $x\notin\mathcal A$, we conclude $\mathcal B^c\subseteq\mathcal A^c$, we proved  \eqref{2020.02.08_10.57}. 
\end{proof}

\begin{lemma}
\label{lem_dons}
 For any measurable function $\phi(\cdot)$, and two distributions $\Prior$ and $\Posterior$, we have
\begin{align}
    \mathbbm E_{\Posterior} [\phi(X)]\leq \Dkl(\Posterior||\Prior)+\log\left(
        \mathbbm E_{\Prior} \left[e^{\phi(X)}\right]
        \right).\label{Donsker}
\end{align}
\end{lemma}
\section{PAC-Bayes Bounds for Meta Learning (unfinished)}
\label{Pac_Bnd_sec}

Since one approach in the meta-learning problem is decomposition approach, having $\func[]{}$ functions satisfying triangle inequality is desirable. Jensen–Shannon divergence satisfies triangle inequality. 
As an example, here, we set
\begin{align}
    \funcTsk[a]{b}=\funcEnv[a]{b}=\JSD[a]{b}=\frac{1}{2}\Dkl(a||\frac{a+b}{2})+\frac{1}{2}\Dkl(b||\frac{a+b}{2}),\label{jsd_f}
\end{align}
where $\JSD[]{}$ denotes the Jensen–Shannon divergence. Generally, we have
\begin{align}
    \JSD[p_1]{p_3}\leq  \JSD[p_1]{p_2}+\JSD[p_2]{p_3}.
\end{align}



In this section, from Corollary \ref{cor1}, we obtain different bounds. Here, we consider   the following assumptions  in Corollary \ref{cor1}:
\begin{itemize}
    \item Set $\func[a]{b}=\JSD[a]{b}$, $\theta_{task}=\lenZm$, $\theta_{\textup{env}}=\lenDataSet$,  $\PriorTsk=\mathrm P_{W|U}$, $\PriorEnv=\mathrm P_{U}$,  loss function bounded on $[\phi_{\min},\phi_{\max}]$    
    \begin{align}
   \JSD[\frac{\empLossEnvRV}{\phi_{\max}}]{\frac{\expLossEnvRV}{\phi_{\max}}} \leq
      \min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} \frac{1}{\lenDataSet}\Dkl\left(\hyperpost||\hyperprior \right)-
     \frac{1}{\lenDataSet}\DAre[\alpha_{\textup{env}}]{\hyperpost}{\hyperprior }\hspace{0em}\nonumber\\
     +\mathbbm E_{\hyperpost}\frac{1}{\lenDataSet\cdot\lenZm}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimU||\mathrm P_{W|U}  \right)-\DAre[\alpha_{\textup{task}}]{\PWcondZimU}{\mathrm P_{W|U} }\right]\nonumber\\
     +\frac{1}{\lenZm}\log\frac{4\lenDataSet\sqrt{\lenZm}}{\delta}
     +\frac{1}{\lenDataSet}\log\frac{4\sqrt{\lenDataSet}}{\delta},
     \label{2021.02.22_01.06}
    \end{align}
    where to bound the last terms in \eqref{eq_B_tsk} and \eqref{eq_B_env}, we follow exactly the same steps presented in \cite{Maurer}.
    \item Applying the inequality $\JSD[a]{b}\geq 0.5(a-b)^2$ to \eqref{2021.02.22_01.06}
    \begin{align}
        \left|\expLossEnvRV-\empLossEnvRV\right|\leq\sqrt{2\phi_{\max}^2}
        \Bigg(
\min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} \frac{1}{\lenDataSet}\Dkl\left(\hyperpost||\hyperprior \right)-
    \frac{1}{\lenDataSet} \DAre[\alpha_{\textup{env}}]{\hyperpost}{\hyperprior }\hspace{0em}\nonumber\\
     +\mathbbm E_{\hyperpost}\frac{1}{\lenDataSet\cdot\lenZm}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimU||\mathrm P_{W|U}   \right)-\DAre[\alpha_{\textup{task}}]{\PWcondZimU}{\mathrm P_{W|U} }\right]\nonumber\\
     +\frac{1}{\lenZm}\log\frac{4\lenDataSet\sqrt{\lenZm}}{\delta}
     +\frac{1}{\lenDataSet}\log\frac{4\sqrt{\lenDataSet}}{\delta}
        \Bigg)^{\frac{1}{2}}
    \end{align}
    \item Set $\func[a]{b}=|a-b|$,
    $\theta_{task}=\lambda_{task}$, $\theta_{\textup{env}}=\lambda_{\textup{env}}$,  $\PriorTsk=\mathrm P_{W|U}$, $\PriorEnv=\mathrm P_{U}$, loss function bounded on $[\phi_{\min},\phi_{\max}]$  
        \begin{align}
        \left|\expLossEnvRV-\empLossEnvRV\right|\leq \min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} \min_{\lambda_{\textup{env}},\lambda_{\textup{task}}\geq 0}
        \frac{1}{\lambda_\textup{env}}\Dkl\left(\hyperpost||\hyperprior \right)-\frac{1}{\lambda_\textup{env}}
     \DAre[\alpha_{\textup{env}}]{\hyperpost}{\hyperprior }\nonumber\\
     +\mathbbm E_{\hyperpost}\frac{1}{\lenDataSet\cdot\lambda_{\textup{task}}}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimU||\mathrm P_{W|U}   \right)-\DAre[\alpha_{\textup{task}}]{\PWcondZimU}{\mathrm P_{W|U} }\right]\nonumber\\
     +\frac{\lambda_{\textup{task}}(\phi_{\max}-\phi_{\min})^2}{8\lenZm}\log\frac{2\lenDataSet}{\delta}
     +\frac{\lambda_{\textup{env}}(\phi_{\max}-\phi_{\min})^2}{8\lenDataSet}\log\frac{2}{\delta}.
        \end{align}
  
        
\end{itemize}



==> textfile/Proof_without_prop-gen-pac.tex <==
\section{Proof of Theorem \ref{without_prop-gen-pac}}
\label{Proof_without_prop-gen-pac}
The proof is very similar to the proof of Theorem \ref{prop-gen-pac-tsk_two_KL} presented in Appendix \ref{Proof_prop-gen-pac-tsk_two_KL}. The main difference here is the way we choose the prior and posterior at the task level. Here, at the task level, for the given task $\task_i$, and  the given hyperparameter $u$, we consider the prior as $\mathrm P_{W_i|U=u}$. Since by observing the samples, the posterior  can be any distribution, we set it as $\mathrm P_{W|\bm Z_i^{\lenZm_i},U=u}$. Next, following exactly the same steps  deriving 
\eqref{pr_tsk_e2}, i.e., setting prior and posterior distributions as $\mathrm P_{W_i|U=u}$ and $\mathrm P_{W|\bm Z_i^{\lenZm_i},U=u}$, respectively, staring from  $\funcTsk[]{}$ of $\expLossTskRV$ and $\empLossTskRV$, then 
applying Jensen's inequality, Donsker-Varadhan theorem, and Markov's inequality, with probability at least $1-\delta_i$ under distribution $\mathrm P_{\trainTsk}$, we have
 \begin{align}
 \funcTsk[ \mathbbm E_{\PWcondZimUsimpSmallU}\left( \mathrm L_{\mathrm P_{Z|\taskRV_i}}(W)  \right)]{  \mathbbm E_{\PWcondZimUsimpSmallU}\left( \empLossTskRV\right)}  %\hspace{12em}\nonumber\\
     \leq   \frac{1}{\theta_{\textup{tsk}}}\Dkl\left(
     \PWcondZimUsimpSmallU||\PriorTskSimpSmallU\right) +\frac{1}{\theta_{\textup{tsk}}}\log\left(
\frac{  \mathbbm E_{\mathrm P_{\taskRV_i\trainTsk}}  \mathbbm E_{    \PriorTskSimpSmallU} e^{\theta_{\textup{tsk}}\funcTsk[ \expLossTskRV]{\empLossTskRV}}}{\delta_i}
     \right). \label{pr_tsk_e_without}
     \end{align}
     
    Next,  by setting $f_i$ and $a_i$ as the left and right hand sides \eqref{pr_tsk_e_without}
    in
    Lemma \ref{Lemma_sum}, with probability at least $1-\sum_i\delta_i$, %under distribution $\mathrm P_{\trainEnv}$,
    we obtain 
    \begin{align}
        \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet
      \funcTsk[ \mathbbm E_{\PWcondZimUsimpSmallU}\left( \mathrm L_{\mathrm P_{Z|\taskRV_i}}(W)  \right)]{  \mathbbm E_{\PWcondZimUsimpSmallU}\left( \empLossTskRV\right)} % \hspace{9em}\nonumber\\
     \leq    \frac{1}{\lenDataSet\cdot\theta_{\textup{tsk}}} \sum_{i=1}^\lenDataSet\Dkl\left(
     \PWcondZimUsimpSmallU||\PriorTskSimpSmallU\right)\hspace{12em}\nonumber\\
     +\frac{1}{\lenDataSet\cdot\theta_{\textup{tsk}}}\sum_{i=1}^\lenDataSet\log\left(
\frac{  \mathbbm E_{\mathrm P_{\taskRV_i\trainTsk}}  \mathbbm E_{    \PriorTskSimpSmallU} e^{\theta_{\textup{tsk}}\funcTsk[ \expLossTskRVRV]{\empLossTskRV}}}{\delta_i}
     \right),  \label{pr_tsk_e_without_2}
    \end{align}
    which holds for any $u\in\mathcal U$.
    Averaging both sides of \eqref{pr_tsk_e_without_2} over $\hyperpost$, setting $\delta_i=\delta/(\kappa\cdot\lenDataSet)$, applying  Jensen's inequality  and using the fact that $\funcTsk[\frac{1}{\lenDataSet}\sum_i^{\lenDataSet} a_i]{\frac{1}{\lenDataSet}\sum_i^{\lenDataSet} b_i}\leq \frac{1}{\lenDataSet}\sum_i^{\lenDataSet}\funcTsk[a_i]{b_i}$,  with probability $1-\delta/\kappa$ under $\mathrm P_{\trainEnv}$, we have
  \begin{align}
      \funcTsk[\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left( \decomMetaRVTot\right)]{\mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \empLossEnvRV}\leq \frac{1}{\lenDataSet}\mathbbm E_{\hyperpost}\left[\sum_{i=1}^\lenDataSet\Ttsk\right],\label{2021.06.14_10.44_a}
  \end{align}
  where $\Ttsk$ is given by \eqref{T_tsk}.
  
  At the environment level, by setting hyper-prior as $\hyperprior$, hyper-posterior as $\hyperpost$, following similar steps derived \eqref{2021.03.10_15.15} (Jensen's inequality,  Donsker-Varadhan theorem), applying and Markov's inequality to \eqref{2021.03.10_15.15}, with probability $1-\delta_0$ under distribution $\mathrm P_{\trainEnv}$, we obtain
  \begin{align}
      \funcEnv[\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left(
\expLossEnvRV
\right)]{\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left( \decomMetaRVTot\right)}\leq \mathrm B_e,
\label{2021.06.14_10.44_b}
  \end{align}
  where $\mathrm B_e$ is given by \eqref{2021.06.14_10.40}.
  
  Finally, like before, we use Lemma \ref{Lemma_sum}. Setting 
  $\lenDataSet=2$, $f_1$ and $a_1$ (resp. $f_2$ and $a_2$)  as the left and right hands  side of \eqref{2021.06.14_10.44_a} (resp. \eqref{2021.06.14_10.44_b}) in Lemma \ref{Lemma_sum}, then  choosing  $\delta_0=(\kappa-1)/\kappa\delta$, we conclude \eqref{cor_without}. Equation \eqref{cor_without_second} is derived by following exactly the same steps. To obtain \eqref{cor_without_second}, firstly we apply $a\leq k_t\cdot b+ \funcinvTsk{c_{\textup{tsk}}}$  and $a\leq k_e\cdot b+\funcinvEnv{c_{\textup{env}}}$ to \eqref{pr_tsk_e_without}  and \eqref{2021.06.14_10.44_b}, and then by following the same steps,  we use Lemma \ref{Lemma_sum}. 

==> textfile/lemma.tex <==
\section{Lemma}
We mainly use the following Lemma.
\begin{lemma}
\label{prior-indep-square}
Let $X_1,...,X_m$ be i.i.d. random variables. Assume $\Delta=\mathbbm E[g(X)]-\frac{1}{m}\sum_{k=1}^mg(X_i)$, where $g(\cdot)$ is sub-Gaussian with parameter $\sigma$. 
Then ,
\begin{align}
    \mathbbm E\left[e^{\lambda m \Delta^2}  \right]\leq \frac{1}{\sqrt{1-2\lambda\sigma^2}}, 
\end{align}
for $\lambda\leq\frac{1}{2\sigma^2}$.
\end{lemma}
\begin{proof}
The proof is similar to \cite[Th. 2.6]{Wainwright}. For completeness, we repeat it again.
Since $g(\cdot)$ is sub-Gaussian, we have
\begin{align}
    \mathbbm E\left[ e^{\lambda\Delta} \right]\leq \exp\left( \frac{\lambda^2\sigma^2}{2m} \right).\label{201.03.16_14.27}
\end{align}
Multiplying both sides of \eqref{201.03.16_14.27} by $\exp(-\frac{\lambda^2\sigma^2}{2sm})$ for $s\in(0,1)$, we find that
\begin{align}
    \mathbbm E\left[ e^{\lambda\Delta-\frac{\lambda^2\sigma^2}{2sm}} \right]\leq \exp\left( \frac{-\lambda^2\sigma^2}{2ms}(-s+1) \right).\label{201.03.16_14.29}
\end{align}
Next, we take integration with respect to $\lambda$. 
Since \eqref{201.03.16_14.29} is valid for any $\lambda\in\mathbbm R$, by using Fubini's theorem, we exchange the order of expectation and integration, leading to
\begin{align}
    \mathbbm E\left[ \exp\left(\frac{s m\Delta^2}{2\sigma^2}\right) \right]\leq \frac{1}{\sqrt{1-s}},\hspace{2em}\textup{for }0<s<1.
\end{align}
By defining $\lambda=\frac{s}{2\sigma^2}$, we conclude the proof.
\end{proof}


==> textfile/main_tool.tex <==
\section{Main Tools for PAC-Bays Bounds}
\label{sec_tool}
In this section, we present  number of propositions and lemmas that work as  the main tools to provide general PAC-Bayes bounds  presented in Theorem \ref{th1_simple} and Proposition \ref{prop-gen-pac-tsk_two_KL}. 
Throughout this section, we assume that the the number of samples in task $\task_i$ is $\lenZm_i$.
\begin{proposition}
\label{prop-gen-pac-tsk}
Let $\lenZm_i$ denotes the the number of samples in task $\task_i$, and let $\funcTsk[a]{b}$ be a function which is convex in both $a$ and $b$. For  prior $\PriorTskSimp$, with probability at least $1-\delta_i$ under $\mathrm P_{\trainTskSimp}$,  we have
\begin{align}
 \funcTsk[\mathbbm E_{\PWcondZimUsimp}(\expLossTskRV)]{\mathbbm E_{\PWcondZimUsimp}(\empLossTskRV)}\hspace{10em}\nonumber\\
 \leq   
 \Dkl\left(\PWcondZimUsimp||\PriorTskSimp \right)
+\log\left(\frac{
\mathbbm E_{\mathrm P_{\trainTskSimp}}\mathbbm E_{\PriorTskSimp}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right).
\label{prop-gen-pac-tsk_formula}
\end{align}
\end{proposition}
\begin{proof}
\begin{align}
       &\funcTsk[\mathbbm E_{\PWcondZimUsimp}(\expLossTskRV)]{\mathbbm E_{\PWcondZimUsimp}(\empLossTskRV)}\\
        %%%%%%%%%%%%%%%%%%%%%%%%%line2
\textup{Jensen's Inequality} \hspace{2em}       &\leq 
\mathbbm E_{\PWcondZimUsimp}\funcTsk[\expLossTskRV]{\empLossTskRV}
\\
        %%%%%%%%%%%%%%%%%%%%%%%%%line3
\textup{Eq. \eqref{Donsker} or \eqref{newOne}}  \hspace{2em} 
   &\leq 
\Dkl\left(\PWcondZimUsimp||\PriorTskSimp \right)
+\log\left(
\mathbbm E_{\PriorTskSimp}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}\right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\line4
\textup{Markiv; w.p. $\geq 1-\delta_i$}\hspace{2em}
&\leq 
\Dkl\left(\PWcondZimUsimp||\PriorTskSimp \right)
+\log\left(\frac{
\mathbbm E_{\mathrm P_{\trainTskSimp}}\mathbbm E_{\PriorTskSimp}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta_i}\right).
\end{align}
\end{proof}
\begin{proposition}
\label{prop-gen-pac-env}
Let $\funcEnv[a]{b}$ be a function which is convex in both $a$ and $b$. For any data-free or data-dependent prior $\PriorEnvSimp$, with probability at least $1-\delta_0$ under $\mathrm P_{\trainEnvSimp}$,  we have
\begin{align}
\funcEnv[\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\big(\expLossEnvRV\big)]{\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\Big(\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV\Big)}\hspace{10em}\nonumber\\
\leq \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left(
\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}
\right)\label{Pr_env1}
\\
 \leq   
 \Dkl\left(\mathrm P_{U|\trainEnvSimp}||\PriorEnvSimp  \right)
+\log\left(\frac{
\mathbbm E_{\mathrm P_{ \trainEnvSimp}}\mathbbm E_{\PriorEnvSimp}\, e^{\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}}}{\delta_0}\right).\label{Pr_env}
\end{align}
\end{proposition}
\begin{proof}
The proof is very similar to the proof of Proposition \ref{prop-gen-pac-tsk}. 
\end{proof}

Next, by combining Propositions \ref{prop-gen-pac-tsk} and \ref{prop-gen-pac-env}, we can obtain  PAC-Bayes bounds for the meta-learning problem. To find such bounds, we need additional tools.
In the following, we present lemmas, which are used to derive PAC-Bayes bounds for the meta-learning problem.
\begin{lemma}
\label{Lemma_sum}
Let $X_i$ for  $i=1,...,\lenDataSet$ be independent random variables. Suppose  that for given $a_i\in\mathbbm R^+$, and  measurable  function $f_i$
\begin{align}
    \mathbbm P_{X_{i}}[f_i(X_i)\geq a_i]\leq \delta_i,\label{2020.08.05_19.45}
\end{align}
where $\delta_i\in[0,1]$. Then, 
\begin{align}
    \mathbbm P_{X_{1:\lenDataSet}}\left[\sum_i f_i(X_i)\leq \sum_i a_i\right]\geq 1-\sum_i\delta_i.\label{2021.02.21_23.11}
\end{align}
\end{lemma}
\begin{proof}
Firstly, we show that
\begin{align}
   \underbrace{ \left\{(x_1,...,x_\lenDataSet):\; \sum_i f_i(x_i)\geq  \sum_i a_i\right\}}_{\mathcal A}\subseteq\underbrace{\bigcup_{i=1}\{x_i:\; f_i(x_i)\geq a_i\}}_{\mathcal B}.\label{2021.02.21_23.12}
\end{align}
Let $(x_1,...,x_\lenDataSet)\notin \mathcal B$. It means that for all $i=1,...,\lenDataSet$, $f_i(x_i)<a_i$ which leads that $\sum_i f_i(x_i)<\sum_i a_i$, or $(x_1,...,x_\lenDataSet)\notin \mathcal A$. Thus, $\mathcal B^c\subset \mathcal A^c$, or equivalently $\mathcal A\subset \mathcal B$.

Next, from \eqref{2021.02.21_23.12}, one can conclude
\begin{align}
    \mathbbm P_{X_{1:\lenDataSet}}\left[\sum_i f_i(X_i)\geqslant \sum_i a_i\right ]\leq
    \sum_i     \mathbbm P_{X_{1:\lenDataSet}}\left[  f_i(X_i)\geqslant  a_i\right ]=    \sum_i     \mathbbm P_{X_{i}}\left[  f_i(X_i)\geqslant  a_i\right ]
    \leq\sum_i\delta_i \label{2020.08.05_19.58}
\end{align}
where the last inequality follows from
\eqref{2020.08.05_19.45}.  The proof can be concluded from \eqref{2020.08.05_19.58}.

\end{proof}


\begin{lemma}
\label{lem_triangle}
Let $\func[]{}$ be a function satisfying the following  inequality
\begin{align}
  \func[x]{y}\leq a_1 \cdot \func[x]{z}+ a_2 \cdot \func[z]{y}, \label{2021.02.21_22.34}
\end{align}
where $a_1$ and $a_2$ are positive coefficient. 
Under probability $\mathrm P_{\trainEnvSimp}$, we have
\begin{align}
    \mathbbm P\left( \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\func[\expLossEnvRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}
        +
        \textup{B}_{\textup{e}}\right)\hspace{5em}\nonumber\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \leq
            \mathbbm P\left(a_1\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\func[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMeta[U]{\bm Z^\lenZm_i}{\task_i}}  \right]\geq        \textup{B}_{\textup{e}}\right)\nonumber\\
            +
                  \mathbbm P\left( a_2\cdot\mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\func[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}\right).
\end{align}
\end{lemma}
\begin{proof}
\begin{align}
       & \mathbbm P\left( \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\func[\expLossEnvRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}
        +
        \textup{B}_{\textup{e}}\right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%line 2
    & \leq
 \mathbbm P\Bigg( a_1\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \bigg[
 \func[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]}\nonumber\\
&\hspace{5em} +
 a_2\cdot\func[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}
 \bigg]\geq \textup{B}_{\textup{t}}
        +
        \textup{B}_{\textup{e}}\Bigg)\label{2021.02.21_22.38}\\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%line 3
        &\leq
                  \mathbbm P\left(a_1\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\func[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMeta[U]{\bm Z^\lenZm_i}{\task_i}}  \right]\geq 
        \textup{B}_{\textup{e}}\right)\nonumber\\
         &\hspace{5em}   +
                  \mathbbm P\left(a_2\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\func[\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV]{\empLossEnvRV}  \right]\geq \textup{B}_{\textup{t}}
\right),\label{2021.02.21_22.41}
\end{align}
where \eqref{2021.02.21_22.38} follows from
\eqref{2021.02.21_22.34}, and the fact that $\mathbbm P[A\geq a]\leq \mathbbm P[B\geq a]$ if $A\leq B$. Equation \ref{2021.02.21_22.41} is a direct result of \eqref{2021.02.21_23.12}, i.e.,
    \begin{align}
        \left\{(x_1,x_2):\;
        f_1(x_1)+f_2(x_2)\geq \textup{B}_\textup{t}+ \textup{B}_\textup{e}
        \right\}\subset
         \left\{x_1:\;
        f_1(x_1)\geq \textup{B}_\textup{t}
        \right\}\bigcup
              \left\{
        x_2:\;
        f_2(x_2)\geq \textup{B}_\textup{e}
        \right\}
    \end{align}
\end{proof}

==> textfile/name.tex <==

In this approach, 
the final bound is expressed as 
\begin{align}
    \funcEnv[\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left(
\expLossEnvRV
\right)]{\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left( \decomMetaRVTotRV\right)}\hspace{10em}\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
+\funcTsk[\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\big( \decomMetaRVTotRV\big)]{\mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \big(\empLossEnvRV\big)}\leq c,
\label{2021.11.04_11.16}
\end{align}




      \begin{align}
\log\left(
\frac{ 2\lenDataSet \mathbbm E_{\mathrm P_{T_{1:\lenDataSet}}}\mathbbm E_{\mathrm P_{\trainEnvSimp|T_{1:\lenDataSet}}}  \mathbbm E_{   \PriorEnvSimp \PriorTskSimp} e^{2(\lenZm-1)\left(\mathrm L_{\mathrm P_{Z|\taskRV_i}}(W)-\empLossTskRV\right)^2}}{\delta}
     \right)\leq \log\left(\frac{2\lenDataSet}{\delta}\right),
     \label{log_tsk_Mc}
     \end{align}
     and
     \begin{align} 
     \log \left(\frac{2\mathbbm E_{\mathrm P_{T_{1:\lenDataSet}}}\mathbbm E_{\mathrm P_{\trainEnvSimp|T_{1:\lenDataSet}}}\mathbbm E_{\PriorEnvSimp}e^{2(\lenDataSet-1\left(
\expLossEnvRV
-\decomMetaRVTotRV\right)^2}}{\delta}\right)\leq\log\left(\frac{2\lenDataSet}{\delta}\right),
\label{log_env_Mc}
\end{align}
where in \eqref{log_tsk_Mc} and \eqref{log_env_Mc}, we used Lemma \ref{useful_lemma}. By setting, $\aTsk=2(\lenZm-1)/\lenZm$ and $\aEnv=2(\lenDataSet-1)/\lenDataSet$, recalling that $\sigma=0.5$, from  \eqref{diff_1_tsk}
and
\eqref{diff_1_env}, we obtained \eqref{log_tsk_Mc} and \eqref{log_env_Mc}.

Now, applying $\funcTsk[a]{b}=2(\lenZm-1)(a-b)^2$ and $\funcEnv[a]{b}=2(\lenDataSet-1)(a-b)^2$ to 


\begin{corollary}
\label{cor_eq_16}
Under setting of Theorem \ref{prop-gen-pac-tsk_two_KL}, let the loss function is bounded on $[0, 1]$, and $\funcTsk[a]{b}=\aTsk(a-b)^2$,  $\funcEnv[a]{b}=\aEnv(a-b)^2$. Then,  \eqref{cor_tup_1} and \eqref{cor_tup_2} are simplified as 
Let $\theta_{\textup{tsk}}=\theta_{\textup{env}}=1$
 \begin{align}
  \mathbbm E_{\mathrm P_{\trainEnvSimp}}\left(\Upsilon_{\textup{tsk}}^{\frac{1}{\lenDataSet}}\cdot
     \Upsilon_{\textup{env}}
\right)   
=
  \mathbbm E_{\mathrm P_{\trainEnvSimp}}\left(\left(  
       \prod_{i=1}^{\lenDataSet}\mathbbm E_{ \JointPriorTskSimp} e^{ 
     \funcTsk[
     \expLossTskRV]{
     \empLossTskRV}}
  \right)^{\frac{1}{\lenDataSet }}\cdot
     \left(\mathbbm E_{\PriorEnvSimp}e^{
\funcEnv[
\expLossEnvRV
]{\decomMetaRVTot}} \right)
\right) \label{comp_1}\\
=  \mathbbm E_{\mathrm P_{\trainEnvSimp}}\left(  
       \prod_{i=1}^{\lenDataSet}\mathbbm E_{ \JointPriorTskSimp} e^{ 
     \funcTsk[
     \expLossTskRV]{
     \empLossTskRV}}
  \right)^{\frac{1}{\lenDataSet }}\cdot
    \mathbbm E_{\mathrm P_{\trainEnvSimp}} \left(\mathbbm E_{\PriorEnvSimp}e^{
\funcEnv[
\expLossEnvRV
]{\decomMetaRVTot}} \right)
\label{comp_2}\\
%%%%%%%%%%%%%%%%%%%%
\leq \left(  \mathbbm E_{\mathrm P_{\trainEnvSimp}}
       \prod_{i=1}^{\lenDataSet}\mathbbm E_{ \JointPriorTskSimp} e^{ 
     \funcTsk[
     \expLossTskRV]{
     \empLossTskRV}}
  \right)^{\frac{1}{\lenDataSet }}\cdot
    \mathbbm E_{\mathrm P_{\trainEnvSimp}} \left(\mathbbm E_{\PriorEnvSimp}e^{
\funcEnv[
\expLossEnvRV
]{\decomMetaRVTot}} \right)
\label{comp_3}
 \end{align}
 \begin{align}
  \left(  \mathbbm E_{\mathrm P_{\trainEnvSimp}}
       \prod_{i=1}^{\lenDataSet}\mathbbm E_{ \JointPriorTskSimp} e^{ 
     \funcTsk[
     \expLossTskRV]{
     \empLossTskRV}}
  \right)^{\frac{1}{\lenDataSet }}\cdot
    \mathbbm E_{\mathrm P_{\trainEnvSimp}} \left(\mathbbm E_{\PriorEnvSimp}e^{
\funcEnv[
\expLossEnvRV
]{\decomMetaRVTot}} \right)
\label{comp_3}\\
=
\left(  
       \prod_{i=1}^{\lenDataSet}\mathbbm E_{ \JointPriorTskSimp}\mathbbm E_{\mathrm P_{\trainTskSimp}} e^{ 
     \funcTsk[
     \expLossTskRV]{
     \empLossTskRV}}
  \right)^{\frac{1}{\lenDataSet }}\cdot
   \left(\mathbbm E_{\PriorEnvSimp}  \mathbbm E_{\mathrm P_{\trainEnvSimp}}e^{
\funcEnv[
\expLossEnvRV
]{\decomMetaRVTot}} \right)
\label{comp_4}
 \end{align}
\end{corollary}


\begin{theorem}
\label{th1_simple}
Let $\funcTsk[a]{b}$ and $\funcEnv[a]{b}$ be two functions which are convex in both $a$ and $b$. 
Additionally,  assume that from   $\funcTsk[a]{b}\leq c_{\textup{tsk}}$ (res.  $\funcEnv[a]{b}\leq c_{\textup{env}}$), we can conclude 
$a\leq k_t\cdot b+ \funcinvTsk{c_{\textup{tsk}}}$ (resp. $a\leq k_e\cdot b+\funcinvEnv{c_{\textup{env}}}$) for $k_t\in\mathbbm R^+$ (resp. $k_e\in\mathbbm R^+$).

Having $\lenDataSet$ independent tasks drawn according $\mathrm P_{\taskRV}$, with probability at least $1-\delta$ under $\mathrm P_{\trainEnv}$,  we have
 \begin{align}
      \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\expLossEnvRV\right]\leq  k_e\cdot k_t\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[\empLossEnvRV
 \right] \hspace{7em}\nonumber\\+k_e\cdot \mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet  \funcinvTsk{\textup{B}_{\textup{task}}}\right]
       +
       \funcinvEnv{ \textup{B}_{\textup{env}}},\label{thr1_sim}
 \end{align}
 where
\begin{align}
 \textup{B}_\textup{task}= 
 \Dkl\left(\PWcondZimU||\PriorTsk  \right)
+\log\left(\frac{\tau\lenDataSet
\mathbbm E_{\mathrm P_{\trainTsk}}\mathbbm E_{\mathrm P_{W|U}}\, e^{\funcTsk[\expLossTskRV]{\empLossTskRV}}}{\delta}\right),\label{b_tsk_simp}
\end{align}
and
\begin{align}
     \textup{B}_\textup{env}=  \Dkl\left(\hyperpost||\hyperprior  \right)
+\log\left(\frac{\tau
\mathbbm E_{\mathrm P_{\trainEnv}}\mathbbm E_{\PriorEnv}\, e^{\funcEnv[\expLossEnvRV]{\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \decomMetaRV}}}{(\tau-1)\delta}\right).\label{b_env_simp}
\end{align}
\end{theorem}

==> textfile/new_bounds.tex <==
\section{New PAC-Bayes Bounds for Meta learning}
\label{our-bounds}
In this section, in view of Corollary \ref{cor1}, we obtain new bounds for the meta-generalization error. We use \eqref{cor1_first} to find bounds.
\begin{itemize}
    \item The loss function is bounded by  $\mathrm L_{\max}$; $\funcEnv[a]{b}=\lenDataSet\Dkl(a,b)$ and $\funcTsk[a]{b}=\lenZm\Dkl(a,b)$ (all $\lenZm_i=\lenZm$ or $\lenZm=\max M_i$):
     \begin{align}
      \lenDataSet\mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[
 \lenDataSet\Dkl\left(\frac{\expLossEnvRV}{\mathrm L_{\max}}\big\|\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet} \frac{\decomMetaRV}{\mathrm L_{\max}}   ]\right)
 +
  \lenZm\Dkl\left(\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}    \frac{\decomMetaRV}{\mathrm L_{\max}}\Big\|\frac{\empLossEnvRV}{\mathrm L_{\max}}\right)
 \right]\nonumber\\\leq \min_{\tau>1} \mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \Dkl\left(\PWcondZimUsimp||\PriorTskSimp \right)
+\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\log\left(\frac{2\tau\lenDataSet\sqrt{\lenZm_i}
}{\delta}\right)\right]
  \nonumber\\      +
\Dkl\left(\mathrm P_{U|\trainEnvSimp}||\PriorEnvSimp  \right)
+\log\left(\frac{2\tau\sqrt{\lenDataSet}
}{(\tau-1)\delta}\right),\label{2021.03.21_10.53}
 \end{align}
 where in \eqref{2021.03.21_10.53}, we used Lemma \ref{kl_lem}.
 
 \item 
 Combining the facts that  $\Dkl(a||b)\geq 2(a-b)^2$ and  $\frac{2\lenDataSet\lenZm}{\lenDataSet+\lenZm}(a-c)^2\leq 2\lenDataSet(a-b)^2+ 2\lenZm(b-c)^2$, we conclude 
 $\frac{2\lenDataSet\lenZm}{\lenDataSet+\lenZm}(a-c)^2\leq \lenDataSet \Dkl(a||b)+\lenZm\Dkl(b||c)$. 
 Inserting this inequality to \eqref{2021.03.21_10.53}, and  recalling  that $(\mathbbm E [A-C])^2\leq \mathbbm E [A-C]^2$, we find that
 \begin{align}
    \left |\mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[
   \expLossEnvRV- \empLossEnvRV \right] \right|
   \leq \min_{\tau>1}\mathrm L_{\max}\frac{\lenDataSet+\lenZm}{2\lenDataSet\lenZm}\Bigg(\Dkl\left(\mathrm P_{U|\trainEnvSimp}||\PriorEnvSimp  \right)
\hspace{5em}\nonumber\\
%%%%%%%%%%
+\log\left(\frac{2\tau\sqrt{\lenDataSet}
}{(\tau-1)\delta}\right)
+\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\left[ \frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet \Dkl\left(\PWcondZimUsimp||\PriorTskSimp \right)
+\frac{1}{\lenDataSet}\sum_{i=1}^\lenDataSet\log\left(\frac{2\tau\lenDataSet\sqrt{\lenZm_i}
}{\delta}\right)\right]
\Bigg)^\frac{1}{2}
 \end{align}
 
 \item Fast rate: 
 \begin{align}
   \mathbbm E_{\mathrm P_{U|\trainEnvSimp}} \left[
   \expLossEnvRV\right]\leq
   \min_{\lambda_e,\lambda_t\geq 0.5}
      \frac{1}{1-\frac{1}{2\lambda_e}}\cdot \frac{\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\empLossEnvRV}{1-\frac{1}{2\lambda_t}}+
 \frac{\log(\frac{2}{\delta})}{{1-\frac{1}{2\lambda_e}}} \left(\lambda_e+ \frac{\lambda_t }{1-\frac{1}{2\lambda_t}}
 \right)\nonumber\\
      \frac{\lambda_e}{1-\frac{1}{2\lambda_e}}\left(
   \Dkl\left( \mathrm P_{U|\trainEnvSimp} \Big\|   \PriorEnvSimp\right) \right)+ 
       \frac{1}{1-\frac{1}{2\lambda_e}}\cdot \frac{\lambda_t}{1-\frac{1}{2\lambda_t}}\left( 
       \Dkl\left(\mathrm P_{UW|\trainEnvSimp}
       \Big\| \mathrm P_{UW}
       \right)
    \right)
 \end{align}
 
\item  Set $\func[a]{b}=|a-b|$,
    $\theta_{task}=\sqrt{\lenZm}$, $\theta_{\textup{env}}=\sqrt{\lenDataSet}$,  $\PriorTsk\propto e^{\gamma_{\textup{task}}\empLossTskRV}$, $\PriorEnvSimp\propto e^{\gamma_{\textup{env}}\empLossEnvRV}$,          \begin{align}
       \expLossEnvRV-\empLossEnvRV\leq \min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} 
        \frac{1}{\sqrt{\lenDataSet}}\Dkl\left(\mathrm P_{U|\trainEnvSimp}||\PriorDataDepEnv[U]{\trainEnvSimp}{} \right)\nonumber\\
     +\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\frac{1}{\lenDataSet\cdot\sqrt{\lenZm}}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimUsimp||\PriorDataDepTsk[W]{\trainTskSimp}{U}  \right)\right]\nonumber\\
     +\frac{2(1+\frac{2\gamma_{\textup{task}}}{\sqrt{\lenZm}})+ \log\frac{2\lenDataSet(1+\sqrt{e})}{\delta}}{\sqrt{\lenZm}}
     +\frac{2(1+\frac{2\gamma_{\textup{env}}}{\sqrt{\lenDataSet}})+ \log\frac{2(1+\sqrt{e})}{\delta}}{\sqrt{\lenDataSet}}.
        \end{align}     
\end{itemize}


==> textfile/short_pre.tex <==
\section{Previous Work}
To have a compact notation, we provide Table \ref{table_notation} to show all mathematical symbols used in this report.
\begin{table}[h]
\begin{center}
\begin{tabular}{ cc }
\vline
\begin{tabular}{*{2}{c}}
\hline
& $\lenZm_i$ ;  Number of samples in the $i$-th task\\
\hline
& $\task$; Realization of task 
\\
\hline
& $j$; Index of task \\
\hline
& $\PZT(\cdot|\task_i)$; Data-set distribution of task $\task_i$ \\
\hline
& $\trainTsk$; Training examples of task $\task_i$ \\
\hline
&$ \decomMeta[u]{\bm Z^\lenZm}{\task}=\DefdecomMeta[u]{\bm Z^\lenZm}{\task}$; Decomposition term\\
\hline
& $\expLossTsk[W]{}= \DefexpLossTsk[W]{Z_i^j}$;\\
&per-task expected loss \\
\hline
& $\empLossTsk[W]{}=\DefempLossTsk$;\\
&per-task empirical loss \\
\hline
& $\genTsk[W]{\trainTsk}=\empLossTsk[W]{}-\expLossTsk[W]{}$; \\
&per-task generalization gap\\
\hline
%& $\bm S_i=(S_{i,1},...,S_{i,\lenZm})$;  $S_{i,j}\sim \textup{Ber}(0.5)$\\
%\hline
%& $\tilde{\bm Z}^{2\lenZm_i}_i$;  Super sample (task level)\\
%\hline
%&$\tilde{\bm Z}^{2\lenZm_i}_i(\bm S_i)$;  Randomly $\lenZm$-training samples\\
% \hline
&$\mathrm P_{W|\bm Z_i^{\lenZm_i}U}$;  The base learner\\
\hline
&$\PriorDataFreeTsk[W]{}{U}$;
Task data-free prior
\\
\hline
&$\PriorDataDepTsk[W]{\bm Z^{\lenZm_i}_i}{U}$;
Task data-dependent prior\\
\hline
&$\PostTsk[W]{\trainTsk}{U}$;
Task posterior distribution
\\
\hline
&$\PriorTsk$; both data-free, data-dependent prior
\\
\hline
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vline
\begin{tabular}{*{2}{c}}
\hline
&$\lenDataSet$; Number of tasks \\
\hline
&$\taskRV$; Task random variable\\
\hline
&$i$; Index of environment\\
\hline
&$\mathrm P_{\taskRV}$; Task distribution\\
\hline
&$\trainEnv$; $\lenDataSet$ data sets\\
\hline
&$ \decomMetaRVTot=\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet} \decomMetaRV$;\\ 
\hline
&$\expLossEnv[U]=\DefexpLossEnv[U]$;\\
&meta-expected loss\\
\hline
&$\empLossEnv[U]=\DefempLossEnv $;\\
&meta-empirical loss\\
\hline
&$\genEnv[U]{\trainEnv}=\empLossEnv[U]{ }-\expLossEnv[U]{}$; \\
&meta-generalization gap\\
\hline
%&$\bm R=(R_1,...,R_{\lenDataSet})$;  
% $R_i\sim \textup{Ber}(0.5)$ \\
%\hline
%&$\supSamp$; Super sample\\
%\hline
%&$\supSamTask$; Randomly $\lenDataSet$ meta training samples\\
%\hline
&$\mathrm P_{U|\bm Z_{1:\lenDataSet}^{\lenZm_1:\lenZm_\lenDataSet}}$; The meta learner\\
\hline
&$\PriorDataFreeEnv[U]{}{}$;
Meta data-free prior
\\
\hline
&$\PriorDataDepEnv[U]{\bm Z^{\lenZm_1:\lenZm_\lenDataSet}_{1:\lenDataSet}}{}$;
Meta data-dependent prior\\
\hline
&$\PostEnv[U]{\trainEnv}{}$;
Meta posterior distribution
\\
\hline
&$\PriorEnv$; both data-free, data-dependent prior
\\
\hline
\end{tabular}
\vline
\end{tabular}
\caption{Mathematical symbols}
\label{table_notation}
\end{center}
\end{table}

Throughout this report, except where stated otherwise, we assumed that the loss function is bounded on $[0,1]$, and thus it is sub-Gaussian with parameter $\sigma=0.5$.
Let $\hyperprior$ be some predefined
hyper-prior distribution. 
In both \cite[Th. 2]{amit2018meta}   and  \cite[Th. 2]{rothfuss2020pacoh},  a tuple of
hypothesis consisting of the shared prior is assumed. 
In  \cite[Th. 2]{amit2018meta}, it was proved that for the priors independent of data, with probability at least $1-\delta$ under $\mathrm P_{\trainEnv}$
\begin{align}
        \mathbbm E_{\hyperpost} [\expLossEnv[U]{}]\leq         \mathbbm E_{\hyperpost} [\empLossEnv[U]{}]+\sqrt{\frac{\Dkl\left(\hyperpost||\hyperprior\right)+\log\frac{2\lenDataSet}{\delta}}{2(\lenDataSet-1)}}
        \nonumber\\+\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\sqrt{\frac{\Dkl\left(\hyperpost||\hyperprior\right)+\mathbbm E_{\hyperpost}\left(\Dkl(\PWcondZimU||\mathrm P_{W|U}) \right)+\log\frac{2\lenDataSet\lenZm_i}{\delta}}{2(\lenZm_i-1)}}.\label{amit_th2}
\end{align}
Additionally, in \cite[Th. 2]{rothfuss2020pacoh}, for the priors independent of data, the meta-generalization error is bounded as
\begin{align}
           \mathbbm E_{\hyperpost} [\expLossEnv[U]{}]\leq         \mathbbm E_{\hyperpost} [\empLossEnv[U]{}]+\min_{\lambda,\beta\geq 0} \left( \frac{1}{\lambda}+\frac{1}{\beta} \right)\Dkl\left(\hyperpost||\hyperprior\right)\nonumber\\
           +\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet} \frac{1}{\beta}\mathbbm E_{\hyperpost}\left(\Dkl(\PWcondZimU||\mathrm P_{W|U}) \right)+C(\delta, \lambda,\beta),\label{rothfuss_th2}
\end{align}
where $C(\delta, \lambda,\beta)=(\frac{\lambda}{8\lenDataSet}+\frac{\lambda}{8\lenZm})-\frac{1}{\sqrt\lenDataSet}\log\delta$ if the loss function is bounded. 

If the
loss function is sub-gamma with variance factor $s_I^2$
and
scale parameter $c_I$
for the data distributions $\mathrm P_{Z|\task_i}$ and $s_{II}^2$, $c_{II}$
 for the task distribution $\mathrm P_T$, the inequality holds with $C(\delta, \lambda,\beta)=\frac{\lambda s_{II}^2}{2\lenDataSet(1-( c_{II}\lambda)/\lenDataSet)}+\frac{\beta s_{I}^2}{2\lenZm(1-( c_{I}\beta)/\lenZm)}-\frac{1}{\sqrt\lenDataSet}\log\delta$.

Finally in \cite[Th.1]{Implicit_Prior}, for the priors independent of data, with probability  at least $1-\delta$ under $\mathrm P_{\trainEnv}$ for $\tau>1$
\begin{align}
        \mathbbm E_{\hyperpost} [\expLossEnv[U]{}]\leq         \mathbbm E_{\hyperpost} [\empLossEnv[U]{}]+\sqrt{\frac{\Dkl\left(\hyperpost||\hyperprior\right)+\log\frac{\tau\lenDataSet}{\delta}}{2(\lenDataSet-1)}}
        \nonumber\\+\frac{1}{\lenDataSet}\sum_{i=1}^{\lenDataSet}\sqrt{\frac{\mathbbm E_{\hyperpost}\left(\Dkl(\PWcondZimU||\mathrm P_{W|U}) \right)+\frac{\tau \lenDataSet}{(\tau-1)\delta}\log(\lenZm_i)}{2(\lenZm_i-1)}}.\label{Implicit_Prior_Th1}
\end{align}


==> textfile/unfinished.tex <==
\section{PAC-Bayes Bounds for Meta Learning (unfinished)}
\label{Pac_Bnd_sec}

Since one approach in the meta-learning problem is decomposition approach, having $\func[]{}$ functions satisfying triangle inequality is desirable. Jensen–Shannon divergence satisfies triangle inequality. 
As an example, here, we set
\begin{align}
    \funcTsk[a]{b}=\funcEnv[a]{b}=\JSD[a]{b}=\frac{1}{2}\Dkl(a||\frac{a+b}{2})+\frac{1}{2}\Dkl(b||\frac{a+b}{2}),\label{jsd_f}
\end{align}
where $\JSD[]{}$ denotes the Jensen–Shannon divergence. Generally, we have
\begin{align}
    \JSD[p_1]{p_3}\leq  \JSD[p_1]{p_2}+\JSD[p_2]{p_3}.
\end{align}



In this section, from Corollary \ref{cor1}, we obtain different bounds. Here, we consider   the following assumptions  in Corollary \ref{cor1}:
\begin{itemize}
    \item Set $\func[a]{b}=\JSD[a]{b}$, $\theta_{task}=\lenZm$, $\theta_{\textup{env}}=\lenDataSet$,  $\PriorTsk=\mathrm P_{W|U}$, $\PriorEnvSimp=\mathrm P_{U}$,  loss function bounded on $[\phi_{\min},\phi_{\max}]$    
    \begin{align}
   \JSD[\frac{\empLossEnvRV}{\phi_{\max}}]{\frac{\expLossEnvRV}{\phi_{\max}}} \leq
      \min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} \frac{1}{\lenDataSet}\Dkl\left(\mathrm P_{U|\trainEnvSimp}||\hyperprior \right)-
     \frac{1}{\lenDataSet}\DAre[\alpha_{\textup{env}}]{\mathrm P_{U|\trainEnvSimp}}{\hyperprior }\hspace{0em}\nonumber\\
     +\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\frac{1}{\lenDataSet\cdot\lenZm}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimUsimp||\mathrm P_{W|U}  \right)-\DAre[\alpha_{\textup{task}}]{\PWcondZimUsimp}{\mathrm P_{W|U} }\right]\nonumber\\
     +\frac{1}{\lenZm}\log\frac{4\lenDataSet\sqrt{\lenZm}}{\delta}
     +\frac{1}{\lenDataSet}\log\frac{4\sqrt{\lenDataSet}}{\delta},
     \label{2021.02.22_01.06}
    \end{align}
    where to bound the last terms in \eqref{eq_B_tsk} and \eqref{eq_B_env}, we follow exactly the same steps presented in \cite{Maurer}.
    \item Applying the inequality $\JSD[a]{b}\geq 0.5(a-b)^2$ to \eqref{2021.02.22_01.06}
    \begin{align}
        \left|\expLossEnvRV-\empLossEnvRV\right|\leq\sqrt{2\phi_{\max}^2}
        \Bigg(
\min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} \frac{1}{\lenDataSet}\Dkl\left(\mathrm P_{U|\trainEnvSimp}||\hyperprior \right)-
    \frac{1}{\lenDataSet} \DAre[\alpha_{\textup{env}}]{\mathrm P_{U|\trainEnvSimp}}{\hyperprior }\hspace{0em}\nonumber\\
     +\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\frac{1}{\lenDataSet\cdot\lenZm}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimUsimp||\mathrm P_{W|U}   \right)-\DAre[\alpha_{\textup{task}}]{\PWcondZimUsimp}{\mathrm P_{W|U} }\right]\nonumber\\
     +\frac{1}{\lenZm}\log\frac{4\lenDataSet\sqrt{\lenZm}}{\delta}
     +\frac{1}{\lenDataSet}\log\frac{4\sqrt{\lenDataSet}}{\delta}
        \Bigg)^{\frac{1}{2}}
    \end{align}
    \item Set $\func[a]{b}=|a-b|$,
    $\theta_{task}=\lambda_{task}$, $\theta_{\textup{env}}=\lambda_{\textup{env}}$,  $\PriorTsk=\mathrm P_{W|U}$, $\PriorEnvSimp=\mathrm P_{U}$, loss function bounded on $[\phi_{\min},\phi_{\max}]$  
        \begin{align}
        \left|\expLossEnvRV-\empLossEnvRV\right|\leq \min_{\alpha_{\textup{env}},\alpha_{\textup{task}}\in[0,1]} \min_{\lambda_{\textup{env}},\lambda_{\textup{task}}\geq 0}
        \frac{1}{\lambda_\textup{env}}\Dkl\left(\mathrm P_{U|\trainEnvSimp}||\hyperprior \right)-\frac{1}{\lambda_\textup{env}}
     \DAre[\alpha_{\textup{env}}]{\mathrm P_{U|\trainEnvSimp}}{\hyperprior }\nonumber\\
     +\mathbbm E_{\mathrm P_{U|\trainEnvSimp}}\frac{1}{\lenDataSet\cdot\lambda_{\textup{task}}}\sum_{i=1}^\lenDataSet \left[  
 \Dkl\left(\PWcondZimUsimp||\mathrm P_{W|U}   \right)-\DAre[\alpha_{\textup{task}}]{\PWcondZimUsimp}{\mathrm P_{W|U} }\right]\nonumber\\
     +\frac{\lambda_{\textup{task}}(\phi_{\max}-\phi_{\min})^2}{8\lenZm}\log\frac{2\lenDataSet}{\delta}
     +\frac{\lambda_{\textup{env}}(\phi_{\max}-\phi_{\min})^2}{8\lenDataSet}\log\frac{2}{\delta}.
        \end{align}
  
        
\end{itemize}




